End-to-End 3D Dense Captioning with Vote2Cap-DETR

3D dense captioning aims to generate multiple captions localized with their associated object regions. Existing methods follow a sophisticated ``detect-then-describe'' pipeline equipped with numerous hand-crafted components. However, these hand-crafted components would yield suboptimal performance given cluttered object spatial and class distributions among different scenes. In this paper, we propose a simple-yet-effective transformer framework Vote2Cap-DETR based on recent popular \textbf{DE}tection \textbf{TR}ansformer (DETR). Compared with prior arts, our framework has several appealing advantages: 1) Without resorting to numerous hand-crafted components, our method is based on a full transformer encoder-decoder architecture with a learnable vote query driven object decoder, and a caption decoder that produces the dense captions in a set-prediction manner. 2) In contrast to the two-stage scheme, our method can perform detection and captioning in one-stage. 3) Without bells and whistles, extensive experiments on two commonly used datasets, ScanRefer and Nr3D, demonstrate that our Vote2Cap-DETR surpasses current state-of-the-arts by 11.13\% and 7.11\% in CIDEr@0.5IoU, respectively. Codes will be released soon.

==> cache/Experiment.tex <==
\section{Experimental Results}
\label{ExperimentalResults}
In this section, we introduce our new dataset and evaluate our ChallenCap in a variety of challenging scenarios. 

\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth]{figures/dataset}
	\caption{Illustration of our capturing system and examples of our dataset. The left shows our capturing system, including four RGB cameras (blue) for sparse-view image sequences and Vicon cameras (red) for marker-based motion capture (partially annotated). The right shows the animated meshes from the rigged character-wise template models with various challenging motions.}
	\label{fig:dataset}
\end{figure}

\myparagraph{ChallenCap Dataset.}
There are existing datasets for 3D pose estimation and human performance capture, such as the Human3.6M\cite{ionescu2013human3} dataset that contains 3D human poses in daily activities, but it lacks challenging motions and template human meshes. The AMASS \cite{AMASS_ICCV2019} dataset provides a variety of human motions using marker-based approach, but the corresponding RGB videos are not provided. 
%
To evaluate our method, we propose a new challenging human motion dataset containing 20 different characters with a wide range of challenging motions such as dancing, boxing, gymnastic, exercise, basketball, yoga, rolling, leap, etc(see Fig.\ref{fig:dataset}). We adopt a 12-view marker-based Vicon motion capture system to capture challenging human motions. Each challenging motion consists of data from two modalities: synchronized sparse-view RGB video sequences and marker-based reference motion captured in an unsynchronized manner. 

\begin{figure}[t]
		\centering
		\includegraphics[width=0.95\linewidth]{figures/comp_methods.pdf}
		\caption{Qualitative comparison. Our results overlay better with the input video frames than the results of other methods.
		}
		\label{fig:comp_methods}
\end{figure}

\begin{table}[t]
	\begin{center}
		\centering
		\caption{Quantitative comparision of several methods in terms of tracking accuracy and template mesh overlay.}
		\label{tab:Comparison}
		\resizebox{0.48\textwidth}{!}{
		\begin{tabular}{l|cccc}
			\hline
			Method      & MPJPE ($mm$)$\downarrow$ & PCK0.5($\%$)$\uparrow$ & PCK0.3$\uparrow$ & mIoU($\%$)$\uparrow$ \\
			\hline
			HMR~\cite{HMR18}         & 154.3  & 77.2   & 68.9   & 57.0 \\
			VIBE~\cite{VIBE_CVPR2020}        & 116.7 & 83.7   & 71.8   & 73.7 \\
			MonoPerfCap~\cite{MonoPerfCap} & 134.7 & 77.4   & 65.6   & 65.5 \\
			Ours        & \textbf{ 52.6}  & \textbf{96.6}   & \textbf{87.4}   & \textbf{83.6} \\
			\hline
		\end{tabular}
		}
		%\vspace{3pt}
	\end{center}
\end{table}


\subsection{Comparison}

Our method enables more accurate motion capture for challenging human motions. For further comparison, we do experiments to demonstrate its effectiveness. We compare the proposed ChallenCap method with several monocular 3D human motion capture methods. 
%
Specifically, we apply MonoPerfCap~\cite{MonoPerfCap} which is based on optimization. We also apply HMR~\cite{HMR18} and VIBE~\cite{VIBE_CVPR2020} where the latter also relies on an adversarial learning framework. For fair comparisons, we fine-tune HMR and VIBE with part of manually annotated data from our dataset.
%
As shown in Fig.\ref{fig:comp_methods}, our method outperforms other methods in motion capture quality. Benefiting from multi-modal references, our method performs better on the overall scale and also gets better overlays of the captured body.

\begin{figure}
		\centering
		\includegraphics[width=0.95\linewidth]{figures/comp_sideview.pdf}
		\caption{Qualitative comparison with side views. Our method maintains projective consistency in the side views while other methods have misalignment errors.
		}
		\label{fig:comp_sideview}
\end{figure}

As illustrated in Fig.\ref{fig:comp_sideview}, we perform a qualitative comparison with other methods on the main camera view and a corresponding side view. The figure shows that the side view results of other methods wrongly estimated the global position of arms or legs. This is mainly because our HybridNet promotes capture results for challenging human motions in the world frame.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/comp_multiview.pdf}
	\caption{Qualitative comparison between ChallenCap (green) and MonoPerfCap (yellow) with reference-view verification. As marked in the figure, MonoPerfCap misses limbs in the reference view.}
	\label{fig:comp_multiview}
\end{figure}

Fig.\ref{fig:comp_multiview} shows the reference view verification results. We capture challenging motions in the main view and verify the result in a reference view with a rendered mesh. The figure shows that even MonoPerfCap gets almost right 3D capture results in the main camera view, the results in the reference view show the misalignments on the limbs of the human body. 


Tab.\ref{tab:Comparison} shows the quantitative comparisons between our method and state-of-the-art methods using different evaluation metrics. We report the mean per joint position error (MPJPE), the Percentage of Correct Keypoints (PCK), and the Mean Intersection-Over-Union (mIoU) results. Benefiting from our multi-modal references, our method gets better performance than optimization-based methods and other data-driven methods.


\subsection{Evaluation} \label{paper:Evaluation}
% Ablation study
We apply two ablation experiments. One verifies that it is more effective to apply the robust optimization stage, the other validates that the diligently-designed network structure and loss functions gain for the challenge human motions by comparing with other network structures.

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/opt.pdf}
	\caption{Evaluation for the optimization stage. The figure shows that our robust optimization stage improves the overlay performance.}
	\label{fig:fig_abla_optimize}
\end{figure}
\begin{table}[tb]
	\begin{center}
		\centering
		\caption{Quantitative evaluations on different optimization configurations.
		}
		\label{tab:optimization}
		%\resizebox{\textwidth}{!}{
		\begin{tabular}{l|c|ccc}
			\hline
			Method         & MPJPE$\downarrow$         & PCK0.5$\uparrow$        & PCK0.3 $\uparrow$         \\
			\hline
			MonoPerfCap   & 134.7         & 77.4          & 65.6          \\
			Ours            & 106.5         & 92.8          & 82.2          \\
			Ours + optimization            & \textbf{52.6} & \textbf{96.6} & \textbf{87.4} \\
			\hline
		\end{tabular}
		%}
		%\vspace{3pt}
	\end{center}
\end{table}

\myparagraph{Evaluation on optimization.}
Tab.\ref{tab:optimization} shows the performance of models with or without the optimization module. The baseline 3D capture method is MonoPerfCap~\cite{MonoPerfCap}. The table demonstrates that whether the robust optimization stage is applied, our method outperforms MonoPerfCap. As illustrated in Fig.\ref{fig:fig_abla_optimize}, the obvious misalignment on the limb is corrected when the robust optimization stage is applied.


\myparagraph{Evaluation on network structure.}
We experiment with several different network structures and loss design configurations, the results are demonstrated in Tab.\ref{tab:ablation_network}. The table shows that even only using sparse-view loss or adversarial loss, our method performs better than the simple encoder-decoder network structure without the attention pooling design. It also outperforms VIBE. When using both sparse-view loss and adversarial loss, our method gets  4\% to 5\% increase for PCK-0.5 and 12 to 32 decrease for MPJPE, compared with using only sparse-view or adversarial loss. The experiment illustrates multi-modal references contribute a lot to the improvement of results as illustrated in Fig. \ref{fig:loss}.

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/loss_new.pdf}
	\caption{Evaluation of our network structure. The figure shows the effectiveness of both of our losses. Note that all experiments are applied with the robust optimization stage. Results of the full pipeline overlay more accurately with the input video frames.
	} 
	\label{fig:loss}
\end{figure}

\begin{table}[t]
	\begin{center}
		\centering
		\caption{Quantitative evaluation of different network structure configurations. Our full pipeline achieves the lowest error.
		}
		\label{tab:ablation_network}
		%\resizebox{\textwidth}{!}{
		\begin{tabular}{l|ccc}
			\hline
			Method                                               & MPJPE   $\downarrow$   & PCK0.5  $\uparrow$        & PCK0.3   $\uparrow$       \\
			\hline
			Encoder-Decoder                                       & 109.1         & 85.7          & 81.5          \\
			VIBE                                                  & 94.2          & 90.2          & 82.0          \\
			Ours  +  $\mathcal{L}_{sv}$                           & 64.3          & 92.5          & 84.1          \\
			Ours  +   $\mathcal{L}_{adv}$                         & 84.6          & 91.2          & 84.1          \\
			Ours  +  $\mathcal{L}_{sv}$ +   $\mathcal{L}_{adv}$   & \textbf{52.6} & \textbf{96.6} & \textbf{87.4} \\
			\hline
		\end{tabular}
		%}
		%\vspace{3pt}
	\end{center}
\end{table}





==> cache/Experiment_backup.tex <==
% pose embedding to motion embedding
% Motion Embedding Module to Motion Embedding Module
% sub-move to sub-action

% to-do
% IJCV
% Dataset 说明数据集存在的价值 与现有数据集存在的不同 和必要性, 并着重说明对3D human capturing的贡献
% Dataset 现在不仅包括2D annotation from competitive sports videos, 还包括增加了 3D sport mocap 
% 删掉other application?

% experiments structure
% -- Sport Dataset Introduction
% 	 -- Diving, gym, boxing, 
% 	 -- Evaluated dataset including ours, FineGym, AQA, pennAction
% -- Motion Capturing[Pose evaluation]
%    -- (ours, pennAction)Metric Evaluation on pose dataset
%       -- add new metric for video clips, like VIBE- PA-MPJPE, MPJPE, PVE, Accel
%    -- Qualitative comparision on 3D dataset
%    -- Qualitative comparision on body capturing
%    -- Metric on body capturing
% -- Action Understanding
%    -- (ours, AQA, FineGym)Metric Evaluation on action parsing
%    -- (ours, AQA)Metric Evaluation on action assessment


% to-do
% dataset
% 1 revision dataset part with all sports
% 2 add sport - motion embedding部分的分析、展示

% of experiments
% 1 VIBE load train -> fine-tune on our sport embedding space
% 2 Compare between VIBE, HMR and ours on our dataset/penAction?

% pose estimation
% 1 add more sport estimated figure
% 2 move application的对比结果到 pose的部分

% Action understanding
% 1 add FineGym evalutation 部分来自FineGym的测试结果，给我们方法的结果
% 2 对比openpose/hr-net直接算FineGym的结果，以及加上我们的pose-embedding的结果

In this section, we evaluate our SportsCap in a variety of challenging scenarios. 
%
We first report a new proposed dataset and the training details of our approach on the utilized datasets, followed by the evaluation of our main technical components, including both qualitative and quantitative comparison with previous state-of-the-art methods on both motion capture and action parsing tasks.
Finally, limitations and discussions regarding our approach are provided.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/mocap.pdf}
	\label{fig:mocap_system}
    \caption{The motion capture system. The structure of dome is shown in the left and the motion capture camera is shown in the bottom right. Our system includes 12 multi-view motion capture cameras. The top right figure shows the motion cap suit with 63 marks. With professional performers, we utilize this system to capture 3D challenging motion of sports.}
\end{figure}

\subsection{Dataset}
% 1. Introduce existing datasets.
% 2. We propose a ... dataset ... called....
% 3. List the novelties/advantages of our dataset.
Many datasets exist for human action analysis, such as the MPII~\citep{andriluka14cvpr} and COCO~\citep{lin2014microsoft} for human pose in daily activities, the PennAction~\citep{Zhang_2013_ICCV} for coarse sport recognition, and the AQA~\citep{Parmar_2019_CVPR} and FineGym~\citep{shao2020finegym} dataset for fine-grained action recognition. 
%
We propose a challenging sports dataset called Sports Motion and Recognition Tasks (SMART) dataset, which contains per-frame action labels, manually annotated pose and action assessment of various challenging sports video clips from professional referees. 
%
We also collect the human pose data in sports activities using a marker-based motion capture system (Fig.~\ref{fig:mocap_system}) to provide pose prior to our Motion Embedding Module. 
%
To our best knowledge, our SMART dataset is the most complete dataset for human motion capture and action analysis for sport video (see Tab. ~\ref{tab:dataset}).

Our SMART dataset consists of both competitive sports and daily exercise videos, including the high jump, competitive diving, uneven bars, balance beam and vault-women in competitive sports, and running, badminton, boxing, and keep-fit in the daily exercise category. 
%
The SMART has 640 videos (110K frames) in total, with per-frame skeleton annotation and sub-motion labels, semantic attribute labels, and action assessment scores for competitive sports. 
%
There are about 450,000 annotated skeletons (in the Openpose 25 joints representation~\citep{cao2018openpose}) with corresponding bounding boxes. 
%
In addition to joint locations, we also annotate the visibility of each joint as three types: visible, labeled but not visible, and not labeled (same as the COCO \citep{lin2014microsoft}). To fulfill our goal of 3D pose estimation and fine-grained action recognition, we collect two types of annotations, i.e. the sub-motions (SMs) and semantic attributes (SAs), as we described in Sec. \ref{sms} and Sec. \ref{sas}. We also include the difficulty scores, the number of valid referees, the execution scores, and the final assessment scores for competitive sports in the SMART dataset. We will share our SMART dataset with the community. 
% \wei{What about daily exercises? daily exercises have no action number or score.}

\begin{table}[t]
	\caption{Comparison between the SMART dataset and existing datasets, including MPII-Pose~\citep{andriluka14cvpr}, Penn Action~\citep{Zhang_2013_ICCV}, COCO~\citep{lin2014microsoft}, AQA~\citep{Parmar_2019_CVPR} and FineGym~\citep{shao2020finegym}, regarding size, per video action labels, pose annotation, action assessment, and pose type. We show the distribution and annotation details of each specific sport of SMART in the bottom of the table.}
	\centering
	\label{tab:dataset}
	\begin{spacing}{1.4}
		\resizebox{\linewidth}{!}{
			\begin{tabular}{lccccccc}
				\hline
				Dataset & \makecell[c]{Video                                                                      \\Clips} & Images & \makecell[c]{Actions \\ per clip} & Pose & \makecell[c]{3D\\mocap} & Assess & Type \\
				\hline
				MPII    & -                  & 25K  & -      & \checkmark & $\times$   & $\times$   & General     \\
				COCO    & -                  & 330K & -      & \checkmark & $\times$   & $\times$   & General     \\
				Penn    & 2K                 & 160K & Single & \checkmark & $\times$   & $\times$   & Sport       \\
				AQA     & 1K                 & 150K & Multi  & $\times$   & $\times$   & \checkmark & Dive        \\
				FineGym & 5K                 & 1.9M & Multi  & $\times$   & \checkmark & $\times$   & Gymnastics  \\
				Ours    & \textbf{5K}                 & \textbf{2.1M} & \textbf{Multi}  & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{Sport}       \\
				\hline
				-       & 640                & 110K & Multi  & \checkmark & 15K        & \checkmark & Dive        \\
				-       & 2K                 & 434K & Multi  & \checkmark & 5K         & \checkmark & Vault-Women \\
				-       & 1K                 & 490K & Multi  & \checkmark & 5K         & \checkmark & UnevenBars  \\
				-       & 1K                 & 704K & Multi  & \checkmark & 2K         & \checkmark & BalanceBeam \\
				-       & -                  & 24K  & Single & \checkmark & 5K         & $\times$   & Hurdling    \\
				-       & -                  & 155K & Single & \checkmark & 2K         & $\times$   & PoleVault   \\
				-       & -                  & 96K  & Single & \checkmark & 3K         & $\times$   & HighJump    \\
				-       & -                  & 4K   & Single & \checkmark & 11K        & $\times$   & Boxing      \\
				-       & -                  & 54K  & Single & \checkmark & 2K         & $\times$   & Badminton   \\
				\hline                                                                                            \\
			\end{tabular}}
	\end{spacing}
\end{table}
	\begin{figure*}
		\centering
		\includegraphics[width=0.82\linewidth]{figures/rs_gallery.pdf}
		\caption{3D human shape recovery results on challenging sport videos. For each type of sport, the top row shows the input images, the middle row shows the recovered body mesh, and the bottom row shows the rendering result of the recovered body from an alternative view.}
		\label{fig:rs_gallery}
	\end{figure*}
% 3d dataset xxxx


\begin{figure*}[htb]
	\centering
	\includegraphics[width=\linewidth]{figures/PCK_Chart.pdf}
    \caption{Cumulative relative variance of our sports dataset explained as a function of the number of pose coefficients. (a) and (b) are the sub-motions of diving with different metrics. `All' refers to use all training data rather than restricted to each semantic pose space. (c) and (d) are general motion embedding of gymnastics and daily sport. PCKs indicates the percentage of correct keypoints (see details in~\citep{andriluka20142d}), and the ratio follows \citep{SMPL:2015}.}
	\label{PCK_Chart}
\end{figure*}


In addition to the annotated video data, we also collect the 3D human pose data using a motion capture system to provide pose motion prior for our Motion Embedding Module. 
%
Specifically, we adopt the Vicon system (a 12 views marker-based motion capture system) to capture the rich human pose sequences and hire 30 athletes and 2 professional fitness instructors as our performers. 
%
The performers move according to the guidelines of the corresponding sports to make sure their body movements cover as more sub-motions of the sports as possible (except the motions that are impossible to execute in the capture environment). 
%
For the generalization purpose, each performer repeats the movements two to five times and the same motion is captured from more than two different subjects. 
%
Since only the relative motion matters, we convert the skeleton results from Vicon to the SMPL pose parameters to avoid the variations imposed by the absolute lengths of bones. 
%
In total, we collect more than 500,000 motion frames of 30 performers covering 9 activities, about 1,000 frames for each performance.

%The MoCap data has xxx(numbers) 3D pose sequences related to these sports to support our 3D motion embedding module, like boxing, keep-fit, and so on.
With the annotated 2D poses and MoCap 3D pose data, we collect the Sports Pose Embedding Spaces according to our motion embedding function (Eq.~\ref{Motion Embedding Module}) and use it as the pose priors for sports videos. Currently, Sports Pose Embedding Spaces provides the priors on 2D joints, 3D joints location, and pose parameters of SMPL for 9 sports, as shown in Tab. \ref{tab:dataset}, and we are planning to add more sports in the near future. Because of the regularity of the human body motion in sports/exercises, the Sports Pose  Embedding  Spaces provides strong prior and regularization to ensure that the generated pose result lies in the corresponding action space. The Sports Pose Embedding  Spaces greatly improves the accuracy and robustness of the 2D/3D pose estimation, human body capturing, action recognition/parsing, and action assessment tasks as described in Sec.~\ref{Motion Embedding Module}.  The Sports Pose Embedding  Spaces data will be included in the SMART dataset.

\begin{figure*}[ht]
	\centering
	\includegraphics[width=\linewidth]{figures/PoseResults.pdf}
	\caption{The gallery and comparison of our experiments on 2D pose estimation. With 2D motion embedding spaces, we show the comparison with fine-tuned HRNet \citep{sun2019deep} (The first column) on SMART dataset. Our results (start from the second column) are more robust and reliable under challenging poses and motion blur.}
	\label{fig:PoseResults}
\end{figure*}
\setlength{\tabcolsep}{4pt}
\begin{table*}[ht]
	\begin{center}
		\centering
		\caption{Ablation study (PCA w/o sub-motion labeling, 50/101/152 ResNet as Backbone, and $\mathcal{L}_{\boldsymbol{\alpha}}$ ($\mathcal{L}_{prior}$)/$\mathcal{L}_{\mathbf{J}}$ ($\mathcal{L}_{data}$) as loss for training. With no $\mathcal{L}_{\boldsymbol{\alpha}}$, we follow \citet{kanazawa2018end} use pose parameters as the variable of $\mathcal{L}_{\mathbf{J}}$ directly.) and comparisons with different methods trained on the same SMART dataset: HRNet \citep{sun2019deep}, SimpleBaseline \citep{xiao2018simple}, HMR \citep{kanazawa2018end}, and VIBE \citep{kocabas2020vibe} of our Motion Embedding Module. We project the recovered 3D joints from HMR and VIBE into image as their keypoint predictions. SM-0 to SM-3 are the sub-motions of our sports (e.g. take-off, twist, somersault, and entry for diving). We use the percentage of correct keypoints (PCK-0.3, PCK-0.5) as our metrics.}
		\label{tab:pose}
		%\resizebox{\textwidth}{!}{
		\begin{tabular}{l|c|c|ccccc|cc}
			\hline
			Method                                                              & PoseSpace & Backbone  & SM-0          & SM-1          & SM-2          & SM-3          & PCK-0.3       & PCK-0.5       \\
			\hline
			HRNet \iffalse\citep{sun2019deep}\fi                                & -         & -         & 83.9          & 81.7          & 82.7          & 86.4          & 83.6          & 87.5          \\
			% CPN\cite{xx}            & Resnet?   & 00.0          & 00.0          & 00.0          & 00.0          & 0.0           & 00.0          \\
			Simple\iffalse\citep{xiao2018simple}\fi                             & -         & ResNet152 & 86.3          & 68.5          & 86.7          & 90.4          & 84.2          & 88.9          \\
			HMR\iffalse\citep{xiao2018simple}\fi                                & -         & ResNet50 & 81.3          & 68.9          & 71.9          & 73.1          & 73.8          & 84.1          \\
			VIBE\iffalse\citep{xiao2018simple}\fi                               & -         & - & 72.0          &    41.9       &    78.7       & 59.4          & 44.1          & 62.4          \\
			\hline
			Ours+$\mathcal{L}_{\mathbf{J}}$                                     & -         & ResNet50  & 69.1          & 60.7          & 76.5          & 71.3          & 70.9          & 86.5          \\
			Ours+$\mathcal{L}_{\boldsymbol{\alpha}}$                            & Semantic  & ResNet50  & 82.9          & 75.6          & 83.1          & 90.3          & 83.6          & 91.5          \\
			Ours+$\mathcal{L}_{\boldsymbol{\alpha}}$+$\mathcal{L}_{\mathbf{J}}$ & Single    & ResNet50  & 81.0          & 80.1          & 82.7          & 89.8          & 83.0          & 92.1          \\
			Ours+$\mathcal{L}_{\boldsymbol{\alpha}}$+$\mathcal{L}_{\mathbf{J}}$ & Semantic  & ResNet50  & 81.3          & 80.4          & 87.6          & 88.8          & 84.8          & 92.4          \\
			Ours+$\mathcal{L}_{\boldsymbol{\alpha}}$+$\mathcal{L}_{\mathbf{J}}$ & Semantic  & ResNet101 & \textbf{87.2} & 82.2          & 88.6          & 90.5          & 87.5          & 94.5          \\
			Ours+$\mathcal{L}_{\boldsymbol{\alpha}}$+$\mathcal{L}_{\mathbf{J}}$ & Semantic  & ResNet152 & 83.6          & \textbf{84.6} & \textbf{91.5} & \textbf{94.0} & \textbf{88.5} & \textbf{96.0} \\
			\hline
		\end{tabular}
		%}
		%\vspace{3pt}
	\end{center}
\end{table*}

\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth]{figures/comp_body}
	\caption{Qualitative comparison with the state-of-the-art human shape recovery methods. (a) The input images. (b), (c), (d) are the results of HMR \citep{kanazawa2018end}, VIBE \citep{kocabas2020vibe}, and SMPLify-X \citep{SMPL-X:2019} respectively.  We fine-tune HMR and VIBE on our training set, and provide the 2D poses of our method for SMPLify-X. (e) our results of SportsCap On SMART dataset.}
	\label{fig:comp_body}
\end{figure}


\subsection{Training Details}
% whereas SMART focuses on sports movements (see Fig.~\ref{fig:PoseResults}). To better train and evaluate our SportsCap, we first construct a new competitive sports video dataset, called the SportsCap Dataset (SMART). Our SMART contains rich poses and semantic action annotations. Fig.~\ref{tab:dataset} compares SMART with existing datasets. 
Our Motion Embedding Module relies on both the fine-grained action labels and pose information, we first train and test the Motion Embedding Module on the SMART dataset as few other datasets provide both information. Then we fix the Motion Embedding Module and train the complete SportsCap on SMART, AQA~\citep{Parmar_2019_CVPR} and FineGym dataset~\citep{shao2020finegym}, for 3D sports motion estimation and action understanding.

We resize image patches that contain the human body at a resolution of 256$\times$256 (using the ground truth bounding box in our SMART dataset and detect the bounding box in AQA \citep{Parmar_2019_CVPR} using \citet{liu2016ssd}). We re-sample the video to 90 frames each. For Motion Embedding Module training, we conduct data augmentation via random rotations ($-45^{\circ}$ to $+45^{\circ}$), random scaling (0.7 to 1.3), and flipping horizontally. For Action Parsing Module training, we also augment the skeleton and pose parameters data for J-, B- and P-Streams, respectively. For J-Stream and B-Stream, we scale the joint positions via interpolation to simulate the far and near camera views. In addition, we randomly mirror the skeleton (to emulate viewing from both sides). For the P-Stream, we also scale the coefficients vector.

We use the Adam optimizer \citep{kingma2014adam}, train the Motion Embedding Module in the first 100 epochs and AMP in the following 50 epochs. We train the complete SportsCap in the last 10 epochs. The learning rates of the 0th, 70th, and 150th epoch are $10^{-3}$, $10^{-4}$, and $10^{-5}$, respectively. We train our SportsCap on 4 NVidia 2080Ti GPUs, and the process takes 10 hours for Motion Embedding Module, 5 hours for Action Parsing Module, and 2.5 hours for the whole SportsCap. Once trained, the network processes the $90\times256\times256$ video data at 0.5s for Motion Embedding Module, 0.05s for Action Parsing Module and 1.0s for the data fetching.

For fair comparisons, we re-train HRNet \citep{sun2019deep} and SimpleBaseline \citep{xiao2018simple} using our SMART dataset. For SCADC \citep{Parmar_2019_CVPR}, C3D-LSTM \citep{parmar2017learning}, C3D-AVG \citep{Parmar_2019_CVPR}, and R2+1D \citep{tran2018closer}, we first pre-train the corresponding networks using the UCF101 dataset \citep{soomro2012dataset} and I3D \citep{sun2019deep} on the Kinetics dataset \citep{sun2019deep}, replace their output or the regression layers with our proposed Semantic Attributes Mapping Block module, and fine-tune Semantic Attributes Mapping Block with our SMART dataset.
% 详细说明对比实验的setting 如何训练其他的网络
% 补充HRNet SimpleBaseline如何训练
% 补充C3D I3D等如何训练
% 补充assessment等如何训练(后面有提及 可以把后面的部分提上来)    

\subsection{Motion Embedding Module Evaluation.}
Our Motion Embedding Module aims to embed the pose motion within a certain sub-move of sports actions into parametric space. It relies on both the sub-move labels and per-frame annotated pose for evaluation, hence we test the Motion Embedding Module on the SMART dataset as few other datasets provide both information. We use the classifier in \citep{hu2019see} to first predict the sub-move label. We observe this technique can achieve high accuracy, and the predicted sub-move label helps the Motion Embedding Module for pose and shape recovery. Tab.~\ref{tab_fineGrain} shows our sub-move classification produces an average accuracy of 96.7\%.

% \begin{figure}[t]
% 	\centering
%     \subfigure[Sample testing of diving]{\includegraphics[width=0.43\linewidth]{figures/tesar.pdf}}
%     \hspace{0.5cm}
%     \caption{(a) Pose estimation on a sample frame in dive video using the top-down method, SimpleBaseline\citep{xiao2018simple}) trained on MPII\citep{andriluka14cvpr} dataset, the bottom-up method, OpenPose\citep{cao2018openpose} on COCO\citep{lin2014microsoft} dataset, and SportsCap on our dataset. Here, We intended to show that without proper datasets, state-of-the-art techniques can easily fail on competitive sports videos. All experiments in Sec.~\ref{ExperimentalResults} still use the same training data. }
% \label{fig:tesar}
% \end{figure}

% ECCV 
% 补充使用同一个PCA pose space与不同sub-motion pose space的对比
% 图片上增加all的曲线
\begin{table}[t]
	%\vspace{3pt}
	\caption{Performance of the fine-grained sub-motion classification using the WS-DAN~\citep{hu2019see} on competitive diving video.}
	\centering
	%\small\addtolength{\tabcolsep}{-2.5pt}
	\label{tab_fineGrain}
	\begin{tabular}{l|ccccc|c}
		\hline
		Method & Take & Twist & Some & Entry & Splash & Avg. \\
		\hline
		WS-DAN & 97.8 & 94.5  & 96.5 & 95.3  & 97.6   & 96.7 \\
		\hline
	\end{tabular}
\end{table}

% \afterpage{

% 	\clearpage
% }

\myparagraph{Ablation experiments on pose estimation.}
\pang{There are two ablation experiments. One experiment verifies that it is more effective to use motion embedding analysis for different motion spaces by comparing PCA analysis in different motion spaces. Another experiment validates the mutual gain between 3D motion capture and fine-grained motion understanding by comparing with the state-of-the-art pose estimation works, which illustrates that mutual gain will make the 2D keypoint projection results more accurate.}
PCA analysis in Fig.~\ref{PCK_Chart} demonstrates that the poses of each sub-motion lay in a low-dimensional parametric space. \pang{As can be seen in the figure, when the number of pose coefficients is the same, if the action is restricted to each semantic pose space, the accuracy of the relative cumulative variance ratio and PCK0.3 results are higher than that under all training data pose space. This proves that motion embedding analysis for different motions is necessary and effective. So }comparison with conducting PCA on the complete action data, we further reduce the space dimension by cooperating with the semantic action labels.

% Fig.~\ref{PCK_Chart} shows that the pose space of each semantic exhibits lower-dimensionality. Tab.~\ref{tab:pose} shows that with semantic pose space, the accuracy increases by 1.8\% on the PCK-0.3 metric. We use the first 12 principal components as basis vectors to represent the pose space of each semantic action. A pose can be viewed as the weighted summation of the basis vectors. We also observe that the semantic sub-action recognition is highly accurate as in Tab.~\ref{tab_fineGrain} and it benefits our semantic-based pose space approach.

%\wei{You need an ablation study to prove that the Sports Pose  Embedding Spaces is helpful to the Motion Embedding Module module!!! Answer: Tab. \ref{tab:pose} with no Loss_theta is this ablation study} 
%\chen{need add analysis on two motion capture methods, HMR and VIBE}
%\wei{ Don't understand, there is no loss_theta in tab2 }
Tab.~\ref{tab:pose} shows the performance of the Motion Embedding Module compared with the state-of-the-art pose estimation work, including the HRNet~\citep{sun2019deep} and the SimpleBaseline~\citep{xiao2018simple}. We also compare with state-of-the-art 3D human shape recovery methods, including the HMR~\citep{HMR} and VIBE~\citep{kocabas2020vibe}. For HMR and VIBE, we project the joints of the recovered 3D human models into images and then use the projected joints as their predicted poses. For a fair comparison, we re-train the HRNet, SimpleBaseline, and et.al. on the SMART dataset. We consider the predicted joints with distance errors less than 0.3 and torso length errors less than 0.5 as the correct predictions (see details in~\citep{andriluka20142d}) and report the percentage of correct keypoints (PCK-0.3 and PCK-0.5) as our metrics. For the classifier, we test ResNet-50, -101, -152 as our backbones and find that about every 50 more layers lead to an above 2\% increase for PCK-0.3. Our approach has the similar performance as HRNet~\citep{sun2019deep} and SimpleBaseline\citep{xiao2018simple} for the take-off pose but can better handle other sub-moves which exhibit more complex occlusion patterns, as shown in Fig.~\ref{fig:PoseResults}. VIBE and HMR perform better on sub-motion 0 (SM-0) which is the preliminary motion of diving while performing worse on sub-motion 1 (SM-1) which is the twist motion. Twisting and other professional motions involve fast rotation and flipping of the body and etc, and our method benefits from the proposed sub-action motion embedding analysis \pang{which has structure constraints by PCA for similar poses in each sub-motion and has real human poses as templates, so our method can achieve higher accuracy.} Our method leads by 4.3$\sim$4.9\% on PCK-0.3, and 7.1$\sim$8.5\% on PCK-0.5, this indicates our approach is more accurate in generating joint locations and the joints are more natural and stable (Fig.~\ref{fig:PoseResults}). Further, there is an approximately 5\% drop in accuracy when trained the Motion Embedding Module without the prior loss provided by Sports Pose  Embedding  Spaces (Ours+$\mathcal{L}_{\boldsymbol{\alpha}}$), demonstrates the effectiveness of the Sports Pose Embedding Spaces.

\myparagraph {Comparison on shape recovery.}
\label{shape capturing experments}
Shape recovery from a single viewpoint image/video is a difficult problem, and it becomes even more challenging for sports because of severe occlusions and motion blur. While our Motion Embedding Module has the ability to accurately recover the human pose, and here we conduct the shape recovery experiments to demonstrate its performance. Tab.~\ref{tab:pose} already shows the quantitative comparison of the 2D poses, and we can see that our method outperforms the state-of-art method.
% moved to previous section
%In this table, VIBE, and HMR all get better results on sub-motion 0 which is preparation motion, and get poor performance on sub-motion 1 which is twist motion. Twist motion is a highly professional action with fast rotation and flipping, out method benefit from the proposed sub-action motion embedding analysis, get higher accuracy on those challenging sports movements. 
% We can see that VIBE, which is more inclined to 3D temporal results, is not as accurate as its predecessor HMR in 2D reprojection. We think this is because VIBE pays more attention to the consistency of the human body shape before the projection of the video clip, and we can see these kinds of results in the qualitative analysis later.

Fig.~\ref{fig:comp_body} qualitatively compares our method with the state-of-the-art 3D shape recovery methods. We fine-tune HMR \citep{HMR} and VIBE \citep{kocabas2020vibe} with our dataset, and provide our results on 2D poses for SMPLify-X \citep{SMPL-X:2019}. In the figure, we show both the recovered human shape rendered at the original and alternative viewpoints.  In Fig.~\ref{fig:comp_body}, we can see that VIBE recovers more accurate 3D human shape although its 2D keypoints accuracy is lower than that of HMR (Tab.~\ref{tab:pose}). For challenging sports movements, i.e. the handspring and somersault, both HMR and VIBE perform poorly while ours achieve much more accurate estimation. Further, our method has the ability to recover the limbs with higher fidelity than HMR and VIBE, as denoted by the colored box. Though the SMPLify-X method provides good 2D keypoint estimations~\ref{tab:pose}, but doesn't produce as good 3D shape results. Our approach outperforms all methods by generating both accurate 2D keypoints and well-matched 3D human shapes.

%In the row with the dotted box, we marked the motion capture results of the foot details by different methods.

\begin{table*}[t]
	\begin{center}
		\centering
		\caption{Action parsing evaluation using state-of-the-art approaches vs. our Action Parsing Module method with joint/joint+bone/joint+bone+pose(coefficients) streams, on the SMART dataset, the FineGym dataset \citep{shao2020finegym}, and the AQA dataset \citep{Parmar_2019_CVPR}. }
		\label{tab:action}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{c|l|ccccc|c}
				\hline
				Dataset              & Method                             & TakeOff       & ArmStand.     & Twist No.     & Some No.      & Position      & Diving No.    \\
				\hline
				\multirow{7}{*}{SMART} & C3D-LSTM\citep{parmar2017learning} & 43.1          & 85.3          & 66.1          & 46.8          & 56.0          & 27.3          \\
				                     & R2+1D\citep{tran2018closer}        & 34.9          & 84.4          & 64.2          & 44.9          & 55.6          & 26.1          \\
				                     & I3D\citep{carreira2017quo}         & 61.5          & 92.7          & 70.6          & 69.7          & 70.6          & 58.6          \\
				                     & Ours+J                             & 85.3          & 97.5          & 78.0          & 82.9          & 75.6          & 65.0          \\
				                     & Ours+J+B                           & 84.1          & 98.6          & 76.8          & \textbf{90.2} & 84.7          & 67.1          \\
				                     & Ours+J+B+P Black-Box               & -             & -             & -             & -             & -             & 78.0          \\
				                     & Ours+J+B+P  Semantic Attributes Mapping Block                   & \textbf{96.4} & \textbf{99.8} & \textbf{89.5} & 86.5          & \textbf{92.6} & \textbf{82.2} \\
				\hline
				\multirow{4}{*}{AQA}
				                     & Nibali\citep{nibali2017extraction} & 74.8          & 98.3          & 78.7          & 77.3          & 79.9          & -             \\
				                     & MSCADC\citep{Parmar_2019_CVPR}     & 78.4          & 97.5          & 84.7          & 76.2          & 82.7          & -             \\
				                     & C3D-AVG\citep{Parmar_2019_CVPR}    & 96.3 & 99.7          & 97.5 & \textbf{96.9} & 93.2 & -             \\
				                     & Ours                               & \textbf{97.5}          & \textbf{99.8} & \textbf{97.9}          & 96.3          & \textbf{94.0}          & -             \\

			

				\hline
			\end{tabular}
		}
		%\vspace{3pt}
	\end{center}
\end{table*}

\begin{table}[t]
    \begin{center}
        \centering
        \caption{Action parsing evaluation using state-of-the-art approaches vs. our method on FineGym dataset }
        \label{tab:FineGym}
        % \resizebox{\textwidth}{!}{
            \begin{tabular}{c|l|cc|c}
                \hline
                Dataset              & Method                             & VT       & UB       & partial Gym288        \\

                \hline
                \multirow{4}{*}{FineGym}
                                     & Random &  16.7         & 6.7        & 0.3                  \\
                                     & ST-GCN     & 19.5          & 13.7          & 11.0                \\
                                     & TRN-2stream     & 31.4 & 83.0          & 42.9          \\
                                     & Ours                               & \textbf{34.2}          & \textbf{85.7} & \textbf{46.9}                     \\

                \hline
            \end{tabular}
        % }
        %\vspace{3pt}
    \end{center}
\end{table}



\subsection{Action Parsing Module Evaluation.} Next, we evaluate the Action Parsing Module module using the outputs of Motion Embedding Module. The multi-stream structure along with SAs of the Action Parsing Module module enables faster convergence. The 2s-AGCN structure (J- and B-Stream only) takes 70 epochs to converge, whereas the multi-stream structure converges after only 50 epochs. With Semantic Attributes Mapping Block, we further accelerate convergence to 10 epochs. The result shows the use of P-Stream (Tab.~\ref{tab:action} row 6) significantly improves the accuracy vs. baseline (Tab.~\ref{tab:action} row 4, 5), even though the accuracy on the somersault attribute drops (Tab.~\ref{tab:action} row 5). This is expected as the network easily focuses only on one attribute without structure like semantic attributes mapping block.

We further conduct experiments to illustrate the benefits of Semantic Attributes Mapping Block over black-box. Specifically, we keep the multi-stream backbone but replace Semantic Attributes Mapping Block with black-box without using attribute loss $\mathcal{L}_{attr}$. The network with Semantic Attributes Mapping Block converges after 10 epochs with the final accuracy of 82.2\% whereas the one with black-box converges after over 30 epoch with the final accuracy of 78.0\%.

\myparagraph{Comparison on action parsing.} \pang{Mid-level sub-action motion embedding analysis and 3D  motion capture also helps action parsing. As shown in Tab.\ref{tab:action}}. We compare the overall action parsing performance of diving with methods including MSCADC \citep{Parmar_2019_CVPR}, C3D-LSTM  \citep{parmar2017learning}, C3D-AVG \citep{Parmar_2019_CVPR}, I3D \citep{carreira2017quo} and R2+1D \citep{tran2018closer}. We compare SportsCap with C3D-LSTM and R2+1D on only SMART for dive number prediction. We did not test on MSCADC, C3D-AVG, and Nibaili \citep{nibali2017extraction} since they do not have the ground truth Dive Number. SportsCap achieves the highest accuracy. \pang{For action parsing, when our method using P stream information, the performance will be much better than not using it, this proves that using the pose coefficient analyzed by motion embedding benefit action parsing a lot}. On the AQA dataset, we also compare SportsCap with Nibaili \citep{nibali2017extraction}. SMART achieves slightly better performance as C3D-AVG and outperforms MSCADC and Nabaili. \pang{This shows that our motion embedding method is not only effective on our dataset but also effective on other datasets with the same pose space.} \pang{As shown in Tab. \ref{tab:FineGym}. On the FineGym dataset, we also do sub-action motion embedding analysis with the help of our 3D motion capture data. It can be seen from the experimental results that our method performs much better on the FineGym dataset than ST-GCN that also uses pose information. This is mainly because our 3D motion capture data and motion embedding analysis can better parse this type of sports motion under specific pose spaces.}

\begin{table}[t]
	\centering
	%\scriptsize\addtolength{\tabcolsep}{0pt}
	\caption{Action assessment comparisons on SMART and AQA dataset \citep{Parmar_2019_CVPR}, and compared with C3D-LSTM \citep{parmar2017learning} and R2+1D\citep{tran2018closer}.}
	%\resizebox{0.55\textwidth}{!}{

	\begin{tabular}{c|l|c|c}
		\hline
		Metric                    & Method   & SMART Dataset & AQA Dataset   \\
		\hline
		\multirow{3}{*}{Sp. Cor.} & C3D-LSTM & 53.7          & 84.9          \\
		                          & R2+1D    & 55.6          & \textbf{89.6} \\
		                          & Ours     & \textbf{61.7} & 86.2          \\
		\hline
	\end{tabular}
	\label{table:Assessment}
\end{table}
\myparagraph{Action Assessment.} 
Here, we further evaluate our approach for overall detailed action assessment using the diving motion, which relies on the dive number for final motion scoring. 
%
Action assessment in diving depends on two independent scores, the difficulty score determined by the dive number, and the execution score representing the quality of the action and the splash. We reuse the extracted spatial-temporal features for action quality assessment. To evaluate the splash, we use a pre-trained C3D block \citep{tran2015learning} on the UCF101 dataset \citep{soomro2012dataset} to extract a 4,096 dimensional feature. We concatenate this feature to our spatial-temporal feature for the final execution score assessment. Instead of treating it as a regression problem, we discretize the score range 0-100 to 49 labels evenly. We use the cross entropy loss Eq.~\ref{cross entropy} and conduct the same training strategy with the SA learning. We train our Motion Embedding Module module on our dataset for pose, while training and testing Action Parsing Module for execution score and final score on our dataset and AQA dataset respectively, Tab.~\ref{table:Assessment} shows the result of the testing results. The reported execution score reaches 61.7\% spearman's rank correlation (Sp. Cor.) \citep{pirsiavash2014assessing}.



\subsection{Limitation and Discussion}
% future work       add NLP in action parsing
As the first trial to explore the problem of joint 3D human motion capture and fine-grained motion understanding from monocular challenging non-daily video input, the proposed SportsCap still owns limitations as follows.

%\myparagraph{Failure case.} 
By tailoring our network for a specific subset of moves, our approach may generate erroneous estimations on degraded images. There are some instances such as when the image does not fall into any of the pre-defined pose categories, some body parts are invisible (e.g, head entry into the water), or incomplete images. We note that baseline algorithms in those cases may perform better as they enforce the final estimation to obey more general pose settings.
%Limitation: 
Our approach, in essence, exploits the semantic action analysis, for human pose estimation. This is different from HRNet~\citep{sun2018integral} or SimpleBaseline~\citep{xiao2018simple} that separately predict individual joints. Consequently, our network, once trained, only tackles specific sports rather than general movements as in prior art. In addition, our approach may generate erroneous estimations for large body parts outside the viewport. Lastly, our method can tolerate common deviations from the standard movement as we purposely add such cases into the dataset. But when an athlete makes rare mistakes, it is difficult for our method to accurately detect and analyze the situation.
%Future work: 
Our current setup assumes a single video stream as input. In sports, it is common practice to show two or more video streams. In the future, we plan to combine multiple streams for a 3D pose/shape task. In addition, general human activities can always be separated into small sub-moves. Hence we plan to extend our work to general-purpose pose estimation through human action decomposition, including to expand our SMART dataset as a more general dataset. Besides, it's also an interesting direction to combine the NLP techniques to provide more natural and detailed illustrations and understanding for action assessment. 

% \begin{figure*}[t]
%     \centering
% 	 \subfigure[Driving a 3D avatar.]{
% 	 	\includegraphics[width=0.45\linewidth]{figures/3DFitting.pdf}
%         \label{fig:3DFitting}
% 	}				
%  	\subfigure[Estimating other sports]{
% 		\includegraphics[width=0.27\linewidth]{figures/OtherSport.pdf}
% 		\label{fig:otherSport}
% 	}
% 	\subfigure[Failure cases]{
% 		\includegraphics[width=0.1599\linewidth]{figures/failureCase2.pdf}
% 		\label{fig:failureCase}
% 	}
%  	\caption{(a) The estimated pose can be used to drive a 3D avatar. We use the same SMPL model inferred from the rest pose as the 3D avatar for both HRNet and our Motion Embedding Module. (b) Extensions of our approach to other sports by training Motion Embedding Module on PennAction\cite{Zhang_2013_ICCV}. (c) Failure cases are caused by missing training data and occlusions/image clipping.}
% \end{figure*}	

% \subsection{Other Applications}
% ECCV
% 补充其他运动的测试图片
% 说明我们的方法在其他运动上的测试情况
% 参考在pennAction上的运动测试

% Based on the pose and action analysis results, we can further conduct action assessment and drive a SMPL \citep{SMPL:2015} model, e.g., for virtual and augmented reality applications. 

% \paragraph{\textbf{Driving a 3D Avatar.}} Our pose estimation method can well handle the complex pose and motion blur problem in the diving action (see Fig.~\ref{fig:PoseResults}). We use our Motion Embedding Module output skeleton to drive a 3D human body and animate the diving action (see Fig.~\ref{fig:3DFitting}). Specifically, we optimize the SMPL~\citep{SMPL-X:2019} using our inferred 2D pose sequences. Our animated 3D human faithfully resembles the diving move with smooth and natural transitions whereas results based on prior art exhibit jitters and unnatural moves.

% \paragraph{\textbf{Other sports.}} Our technique can be potentially extended to process other types beyond diving, e.g., by training on the PennAction datasets. Fig.~\ref{fig:otherSport} shows sample results using SAMB for pose estimation on figure skating and gymnastics. However, unlike diving, we have not yet constructed the corresponding datasets with all sub-action labels and scores and therefore we cannot yet perform additional tasks such as auto-scoring and action parsing. 

==> cache/Experiment_manu.tex <==
\section{Experimental Results}
\label{ExperimentalResults}
In this section, we report our new dataset and evaluate our ChallenCap on a variety of challenging scenarios. 

%pang anqi
\begin{figure}[htb]
	\centering
	\includegraphics[width=\linewidth]{figures/dataset}
	\caption{The capturing system and some examples of our dataset. The left shows our capturing system, including four RGB cameras (Blue) for sparse-view image sequences and 12 Vicon Cameras (Red) for marker-based motion capture (partially annotated in the figure). The right shows the animated meshes, from the rigged template models with various captured motions.}
	% We scan these template model with a multi-view stereo system.
	\label{fig:dataset}
\end{figure}

\myparagraph{ChallenCap Dataset.}
There exist datasets for 3D pose estimation and human performance capture, such as the Human3.6M\cite{ionescu2013human3} dataset, which contains 3D human poses in daily activities but lacks challenging motions and can not provide template human meshes. The AMASS \cite{AMASS_ICCV2019} dataset provides a variety of human motions using marker-based motion capture, but the corresponding RGB videos are not provided. 
%
We propose a challenging human motion capture dataset. It contains 20 different characters with a wide range of challenging motions such as dancing, boxing, gymnastic, push-ups, rolling, lying, leap, pike, etc(see Fig.\ref{fig:rs_gallery}). We adopt the 12-view marker-based Vicon motion capture system to capture challenging human motion sequences. Each challenging motion is composed of two modals of data: one is the 4-view RGB video sequences captured by synchronized sparse view cameras, the other is the marker-based reference data that is temporally unsynchronized. 

\begin{figure}[t]
		\centering
		\includegraphics[width=0.95\linewidth]{figures/comp_methods.pdf}
		\caption{Qualitative comparison between ChallenCap and state-of-the art methods. ChallenCap has better overlay performance than the others.
% 		The comparison shows that HMR and VIBE encountered some scale problems or camera view problems. MonoPerfCap encountered misalignment of limb problems.
		}
		\label{fig:comp_methods}
\end{figure}

\begin{table}[t]
	\begin{center}
		\centering
		\caption{Quantitative comparison between our method and state-of-the-art methods. ChallenCap outperforms all previous temporal methods on all four evaluation metrics}
		\label{tab:Comparison}
		\resizebox{0.48\textwidth}{!}{
		\begin{tabular}{l|cccc}
			\hline
			Method      & MPJPE ($mm$)$\downarrow$ & PCK0.5($\%$)$\uparrow$ & PCK0.3$\uparrow$ & mIoU($\%$)$\uparrow$ \\
			\hline
			HMR~\cite{HMR18}         & 154.3  & 77.2   & 68.9   & 57.0 \\
			VIBE~\cite{VIBE_CVPR2020}        & 116.7 & 83.7   & 71.8   & 73.7 \\
			MonoPerfCap~\cite{MonoPerfCap} & 134.7 & 77.4   & 65.6   & 65.5 \\
			Ours        & \textbf{ 52.6}  & \textbf{96.6}   & \textbf{87.4}   & \textbf{83.6} \\
			\hline
		\end{tabular}
		}
		%\vspace{3pt}
	\end{center}
\end{table}


\subsection{Comparison}
%pang anqi
Our method has the ability to accurately capture challenging human motions. Here we conduct the capturing experiments to demonstrate its performance. The proposed ChallenCap technique has been compared to three methods that are able to capture 3D human motion by using a single RGB camera. 
%
The first one is MonoPerfCap~\cite{MonoPerfCap} which is an optimization method, we also compare HMR~\cite{HMR18} and VIBE~\cite{VIBE_CVPR2020} where VIBE also relies on an adversarial learning framework. 
% For fair comparisons, We fine-tune HMR and VIBE with some annotated data from our dataset \textcolor{red}{[Ma: Why some?]}. 
% For VIBE fine-tuning, we annotate some multi-view 3D pose ground truth and combine our marker-based motion sequences with AMASS dataset to fine-tune the VIBE method.

As illustrated in Fig.\ref{fig:comp_methods}. For the 3D human capturing qualities, our method outperforms other state-of-the-art methods. Benefiting from the multi-modal references, our method has a better effect on the overall scale and also gets better details of the captured body.

\begin{figure}
		\centering
		\includegraphics[width=0.95\linewidth]{figures/comp_sideview.pdf}
		\caption{Qualitative comparison between ChallenCap and state-of-the art methods with side view. ChallenCap outperforms others.
% 		Each camera view row is followed by the side view rendering results. The state-of-the-art method gets slightly worse capture on camera view than ours, on the side views there are huge misalignments of limbs for their methods.
		}
		\label{fig:comp_sideview}
\end{figure}

As illustrated in Fig.\ref{fig:comp_sideview}, it shows a qualitative comparison of the main camera view and  corresponding side view with other methods. The picture shows that even other state-of-the-art methods get almost right 3D capture results on the main camera view, their side view results show that they wrongly estimated the position of arms or legs of the human body. This is mainly because our HybridNet boosts the capture results for challenging human motions.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/comp_multiview.pdf}
	\caption{Qualitative comparison between ChallenCap (green) and MonoPerfCap (yellow) using multi-view rendering verification. As marked in the figure, MonoPerfCap misses limbs on the verify view.}
	\label{fig:comp_multiview}
\end{figure}

Fig.\ref{fig:comp_multiview} shows the multi-view rendering verification results. We captured the human motion on a main view and verified the result on another camera view with a rendered mesh. We can see from the comparison that MonoPerfCap failed to get reasonable and complete results compared to our method.



Tab.\ref{tab:Comparison} shows the quantitative comparisons between our method and state-of-the-art methods using different evaluation metrics. We report the mean per joint position error (MPJPE), the Percentage of Correct Keypoints (PCK) and the Mean Intersection-Over-Union (mIoU) results. ChallenCap outperforms all previous methods on the challenging human motions. We can see from the table that benefiting from our multi-modal references, our method gets better performance than optimization-based methods and other data-driven methods.
% Note that for fair comparison, VIBE and HMR are trained on Human3.6M\cite{ionescu2013human3} which is the indoor setting and has minimal background variation the same as our indoor setting.

% Comparison

% Metric: ?
% The state-of-the-arts: HMR MonoPerfCap VIBE ours   more?
% Datasets: our datasets






% \begin{figure}[t]
% 	\begin{minipage}{0.19\linewidth}
% 		\centerline{\includegraphics[width=1\textwidth]{figures/comp_sideview_1.pdf}}
% 		\centerline{Input}
% 	\end{minipage}
% 	\begin{minipage}{0.19\linewidth}
% 		\centerline{\includegraphics[width=1\textwidth]{figures/comp_sideview_2.pdf}}
% 		\centerline{HMR}
% 	\end{minipage}
% 	\begin{minipage}{0.19\linewidth}
% 		\centerline{\includegraphics[width=1\textwidth]{figures/comp_sideview_4.pdf}}
% 		\centerline{VIBE}
% 	\end{minipage}
% 	\begin{minipage}{0.19\linewidth}
% 		\centerline{\includegraphics[width=1\textwidth]{figures/comp_sideview_3.pdf}}
% 		\centerline{MonoPerfCap}
% 	\end{minipage}
% 	\begin{minipage}{0.19\linewidth}
% 		\centerline{\includegraphics[width=1\textwidth]{figures/comp_sideview_5.pdf}}
% 		\centerline{Ours}
% 	\end{minipage}
% 	\caption{Qualitative comparison between ChallenCap and state-of-the art method with side view. Each camera view row is followed by the side view rendering results. We can see from the side view results, even the state-of-the-art method get only slightly worse capture on camera view than ours, on side view there are misalignment of limbs for their methods.}
% 	\label{fig:comp_sideview}
% \end{figure}


\subsection{Evaluation} \label{paper:Evaluation}
% Ablation study
\myparagraph{Evaluation on optimization.}
% 1 rough 3D baseline (MonoPerfCap)
% 2 rough 3D baseline + temporal optimization
% 3 our pipeline without optimization module 
% 4 our pipeline with optimization module 
% show curve, results and table
\begin{figure}[tb]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/opt.pdf}
	\caption{Evaluation for our optimization stage. The figure shows that the optimization stage improves the overlay performance.}
	\label{fig:fig_abla_optimize}
\end{figure}
\begin{table}[tb]
	\begin{center}
		\centering
		\caption{Quantitative evaluations on different optimization configurations.
% 		We experiment with different temporal optimization configurations and compare our method to our baseline method MonoPerfCap. The temporal optimization module provides consistent improvements over the baseline method and our method
		}
		\label{tab:optimization}
		%\resizebox{\textwidth}{!}{
		\begin{tabular}{l|c|ccc}
			\hline
			Method         & MPJPE$\downarrow$         & PCK0.5$\uparrow$        & PCK0.3 $\uparrow$         \\
			\hline
			MonoPerfCap   & 134.7         & 77.4          & 65.6          \\
			Ours            & 106.5         & 92.8          & 82.2          \\
			Ours + optimization            & \textbf{52.6} & \textbf{96.6} & \textbf{87.4} \\
			\hline
		\end{tabular}
		%}
		%\vspace{3pt}
	\end{center}
\end{table}
% \myparagraph{Evaluation on network structure.}
% 1 vibe + optimization
% 2 cvpr19
% 3 (encoder-decoder) + optimization
% 4 our structure no Vicon loss
% 5 our structure no sparse-view loss
% 6 our final
% show curve, results and table
We do two ablation experiments. One verifies that it is more effective to use the optimization stage for our method, the other validates that the diligently-designed network structure and loss function gain for the challenge human motions by comparing with the state-of-the-art network structures.

Tab.\ref{tab:optimization} shows the performance of models with and without the optimization module. The baseline 3D capture method is MonoPerfCap~\cite{MonoPerfCap}. The table demonstrates that regardless of whether the temporal optimization module is applied, our method outperforms MonoPerfCap. As illustrated in Fig.\ref{fig:fig_abla_optimize}, when the optimization module is applied, the obvious errors on the limb was corrected.


\myparagraph{Evaluation on network structure.}
We experiment with several different network structures and loss design configurations and compare our method to state-of-the-art methods, the results are demonstrated in Tab.\ref{tab:ablation_network}. The table shows that even only using sparse-view loss or discriminator loss, our method performs better than the simple encoder-decoder network structure without attention pooling design. It also outperforms VIBE. When using both sparse-view loss and discriminator loss, our method will get  4\% to 5\% increase for PCK-0.5 and 12 to 32 decrease for MPJPE, compared with using only sparse-view loss or applying only discriminator loss. The experiment illustrates multi-modal references contribute a lot to the improvement of results as illustrated in Fig. \ref{fig:loss}.

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.95\linewidth]{figures/loss_new.pdf}
	\caption{Evaluation of our network structure. The figure shows the effectiveness of both of our losses. Note that all experiments configured that the optimization stage is applied. Our final result shows our final result with both losses and the optimization step.
	} %\textcolor{red}{[Ma: Is the final result also processed by the optimization step? Or just processed by both our losses? Make sure we have only one variable for each comparison.]}
	\label{fig:loss}
\end{figure}

\begin{table}[t]
	\begin{center}
		\centering
		\caption{Quantitative evaluation of different network structure configurations.
% 		We experiment with several models using different network structures. The ablation experiment result indicates our method outperformed state-of-the-art methods. And when using sparse-view loss and discriminator loss together as our final experiment, we get the best performance.
		}
		\label{tab:ablation_network}
		%\resizebox{\textwidth}{!}{
		\begin{tabular}{l|ccc}
			\hline
			Method                                               & MPJPE   $\downarrow$   & PCK0.5  $\uparrow$        & PCK0.3   $\uparrow$       \\
			\hline
			Encoder-Decoder                                       & 109.1         & 85.7          & 81.5          \\
			VIBE                                                  & 94.2          & 90.2          & 82.0          \\
			Ours  +  $\mathcal{L}_{sv}$                           & 64.3          & 92.5          & 84.1          \\
			Ours  +   $\mathcal{L}_{adv}$                         & 84.6          & 91.2          & 84.1          \\
			Ours  +  $\mathcal{L}_{sv}$ +   $\mathcal{L}_{adv}$   & \textbf{52.6} & \textbf{96.6} & \textbf{87.4} \\
			\hline
		\end{tabular}
		%}
		%\vspace{3pt}
	\end{center}
\end{table}
% old references:
% 	Metric:   2D metric (PCK)
% 	          3D metric (accel)
% 	          3D metric (acc)
% 	          3D metric (pose with none global RT)

% 	1 Openpose+ManoperCap(our init)
% 	2 Openpose+ManoperCap+Optimization (temporal only)
% 	3 Openpose+ManoperCap+HybridModule (temporal + prior (no 2D supervise finally))

% 	4 Openpose+ManoperCap+HybridModule(st-gcn)+Optimization
% 	5 Openpose+ManoperCap+HybridModule(different net structure2)+Optimization
% 	6 Openpose+ManoperCap+HybridModule(final net structure3)+Optimization (temporal + prior + 2D supervise)

% 	7 Alphapose+ManoperCap+HybridModule(final net structure3)+Optimization (temporal + prior + 2D supervise)

% 	Analysis
% 	(1) 126 shows our basic modules, better than ManoperCap.  better than temporal-based methods
% 	(2) 36 shows our hybrid module can give a huge improvement on pose fixing (a great pose correcter)
% 	(3) 456 shows our network structure achieve great performance on pose correction.
% 	(4) (not that important) 67 shows our network can handle - support different pose approach or types.

% more ?




==> cache/Intro.tex <==
\section{Introduction}
% 1. Marker-less mocap is important
The past ten years have witnessed a rapid development of markerless human motion capture~\cite{Davison2001,hasler2009markerless,StollHGST2011, wang2017outdoor}, which benefits various applications such as immersive VR/AR experience, sports analysis and interactive entertainment.

%With the recent popularity of virtual and augmented reality (VR and AR), there has been a growing demand for reliable 3D human motion capture. As a low-cost alternative to the widely used marker-based solutions, markerless video-based motion capture alleviates the need for intrusive body-worn motion markers and has received increased attention over the last years. 

\begin{figure}[tbp] 
	\centering 
	\includegraphics[width=0.9\linewidth]{figures/fig_1_teaser.pdf} 
	\caption{Our ChallenCap approach achieves robust 3D capture of challenging human motions from a single RGB video, with the aid of multi-modal references.} 
	\label{fig:fig_1_teaser} 
	\vspace{-8pt} 
\end{figure} 


% 2. Issues of existing methods
% 2.1 multi-view solutions
Multi-view solutions~\cite{StollHGST2011,liu2013markerless,joo2015panoptic,collet2015high,TotalCapture, suo2021neuralhumanfvv} achieve high-fidelity results but rely on expensive studio setup which are difficult to be deployed for daily usage.
% 2.2 monocular setting --> pose detector, mocap methods: specific challenging motions, complex motion patterns and severe self-occlusion
Recent learning-based techniques enables robust human attribute prediction from monocular RGB video~\cite{hmrKanazawa17,VIBE_CVPR2020,TEX2SHAPE_2019ICCV,DeepHuman_2019ICCV,PIFuHD}.
%
The state-of-the-art monocular human motion capture approaches~\cite{LiveCap2019tog,MonoPerfCap,EventCap_CVPR2020} leverage learnable pose detections~\cite{OpenPose,Mehta2017} and template fitting to achieve space-time coherent results.
%
However, these approaches fail to capture the specific challenging motions such as yoga or rolling on the floor, which suffer from extreme poses, complex motion patterns and severe self-occlusion under the monocular setting. 

% 2.3 marker-based Vicon: solved, good reference, but hard to transfer
Capturing such challenging human motions is essential for many applications such as training and evaluation for gymnastics, sports and dancing. 
%
Currently, optical marker-based solutions like Vicon~\cite{VICON} are widely adopted to capture such challenging professional motions.
%
However, directly utilizing such marker-based reference into markerless capture is inapplicable since the actor needs to re-perform the challenging motion which is temporally unsynchronized to the maker-based capture. 
%\textcolor{red}{[Ma: Since we also use marker-based reference, do we have the same limitation?]}
% 2.4 VIBE, use AMASS: general prior, not for specific challenging motions
Some data-driven human pose estimation approaches~\cite{HMR18,VIBE_CVPR2020} utilize the unpaired reference in an adversarial manner, but they only extract general motion prior from existing motion capture datasets~\cite{Ionescu14a,AMASS_ICCV2019}, which fails to recover the characteristics of specific challenging motion.
% 2.5 DeepCap: light-weight multi-view reference, rely on per-performer training 
% Intert Video: solve temporal mis-alignment.     
The recent work~\cite{DeepCap_CVPR2020} inspires to utilize the markerless multi-view reference in a data-driven manner to provide more robust 3D prior for monocular capture.
%
However, this method is weakly supervised on the input images instead of the motion itself, leading to dedicated per-performer training. 
%\textcolor{red}{[Ma: Again, since we also use markerless reference, do we have the same limitation? ]}
%
Moreover, researchers pay less attention to combine various references from both marker-based systems and sparse multi-view systems for monocular challenging motion capture. 


% 3. Our key novelty
In this paper, we tackle the above challenges and present \textit{ChallenCap} -- a template-based monocular 3D capture approach for challenging human motions from a single RGB video, which outperforms existing state-of-the-art approaches significantly (See Fig.~\ref{fig:fig_1_teaser} for an overview).
%
Our novel pipeline proves the effectiveness of embracing multi-modal references from both temporally unsynchronized marker-based system and light-weight markerless multi-view system in a data-driven manner, which enables robust human motion capture under challenging scenarios with extreme poses and complex motion patterns, whilst still maintaining a monocular setup.

%to eliminate the inherent orchestrated self-scanning constraint of single-view capture, we first combine the data-driven implicit occupancy representation and the volumetric fusion within a completion optimization pipeline to generate an initial complete human model with fine geometric details.
% Such complete model is utilized to initialize both the performance capture parameters and the associated human priors.
% To enable robust tracking, based on both the initial complete model and the various visual cues, a novel performance capture scheme is proposed to combine the non-rigid tracking pipeline with human pose, shape and parsing priors, through a hybrid and flip-flop motion optimization and an effective material-dependent volumetric fusion strategy.
% Our hybrid optimization not only handles challenging fast human motions but also owns the reinitialization ability to recover from tracking failures and the disappear-reoccur scenarios, while the volumetric fusion strategy estimates material-dependent motion tracking behavior to achieve robust and precise geometry update and avoid deteriorated fusion model caused by challenging fast motion and self-occlusion.



% 4. Our technical pipeline
% 4.1 all utilized references, motion characteristics
More specifically, we introduce a novel learning-and-optimization framework, which consists of a hybrid motion inference stage and a robust motion optimization stage. 
% 4.2 hyrbid motion inference
Our hybrid motion inference utilizes both the marker-based reference which encodes the accurate spatial motion characteristics but sacrifices the temporal consistency, as well as the sparse multi-view image reference which provides pair-wise 3D motion priors but fails to capture extreme poses.
%
To this end, we first obtain the initial noisy skeletal motion map from the input monocular video.
%
Then, a novel generation network, HybridNet, is proposed to boost the initial motion map, which utilizes a temporal encoder-decoder to extract local and global motion details from the sparse-view reference, as well as a motion discriminator to utilize the unpaired marker-based reference.
% 4.3 challenCap dataset
% To train our HybridNet, a new dataset with rich references modalities and various challenging motions is introduced.
% 4.4 robust motion optimization
Besides the data-driven 3D motion characteristics from the previous stage, the input RGB video also encodes 
reliable motion hints for those non-extreme poses, especially for the non-occluded regions.
%
Thus, a robust motion optimization is further proposed to refine the skeletal motions and improve the tracking accuracy and overlay performance, which jointly utilizes the learned 3D prior from the supervised multi-modal references as well as the reliable 2D and silhouette information from the input image reference.
% 5. Our technical contributions: framework; hybrid motion inference+robust motion optimization; dataset
To summarize, our main contributions include: 
\begin{itemize} 
\setlength\itemsep{0em}
	\item We propose a monocular 3D capture approach for challenging human motions, which utilizes multi-modal reference in a novel learning-and-optimization framework, achieving significant superiority to state-of-the-arts. 
	%\textcolor{red}{[Ma: "which utilizes multi-modal reference in a learning-and-optimization framework" seems redundant because we have detailed description in the second contribution.  ]}
	
	\item We propose a novel hybrid motion inference module to learn the challenging motion characteristics from the supervised references modalities, as well as a robust motion optimization module for accurate tracking.
	
	\item We introduce and make available a new challenging human motion dataset with both unsynchronized marker-based and light-weight multi-image references, covering 60 kinds of challenging motions and 20 performers with 120k corresponding images.
	%\textcolor{red}{[Ma: Will we open the dataset if this paper has been accepted?  ]}
\end{itemize} 



==> cache/M_1.tex <==
\section{Approach}
%We first introduce the preprocessing of rough motion input and details of hybrid motion module, then propose the batch motion optimization for final pose sequences.
\subsection{Hybrid Motion Inference} \label{sec:mot_inference}


\myparagraph{Preprocessing.} 
Given an input monocular image sequence $I_t, t\in[1,T]$ of length $T$ and a well-scanned template model,
we first adopt the off-the-shelf template-based motion capture approach~\cite{MonoPerfCap} to obtain the initial skeletal motion $\textbf{S}_t$ and transform it into quaternions format, denoted as $\textbf{Q}^{init}_t$.
% 
More specifically, we only adopt the 2D term from \cite{MonoPerfCap} using OpenPose~\cite{OpenPose} to obtain 2D joint detections. 
%
Please refer to \cite{MonoPerfCap} for more optimization details.
%
Note that such initial skeletal motions suffer from severe motion ambiguity since no 3D prior is utilized, as illustrated in the pre-processing stage in Fig.~\ref{fig:overview}.
%
After the initial optimization, we concatenate the $\textbf{Q}^{init}_t$ and the detection confidence from OpenPose~\cite{OpenPose} for all the $T$ frames into a motion map $\mathcal{Q}\in\mathbb{R}^{T\times 4N_J}$ as well as a confidence map $\mathcal{C}\in\mathbb{R}^{T\times N_J}$. 


%% --------------------------------------------------------------
%% --------------------------------------------------------------

\myparagraph{HybridNet Training.}
Based on the initial noisy motion map $\mathcal{Q}$ and confidence map $\mathcal{C}$, we propose a novel generation network, HybridNet, to boost the initial capture results for challenging human motions.

%
As illustrated in Fig.~\ref{fig:fig_3_network}, our HybridNet learns the challenging motion characteristics by the supervision from multi-modal references.
%
To avoid tedious 3D pose annotation, we utilize the supervision from the optimized motions using sparse multi-view image reference.
%
Even though such sparse-view reference still cannot recover all the extreme poses, it provides rich pair-wise overall 3D motion prior. 
%
To further extract the fine challenging motion details, we utilize adversarial supervision from the marker-based reference since it only provides accurate but temporally unsynchronized motion characteristics due to re-performing. 
%
To this end, we utilize the well-known Generative Adversarial Network (GAN) structure in our HybridNet with the generative network $\mathcal{G}$ and the discriminator network $\mathcal{D}$.

% 1. sparse-view reference
Our generative module consists of a global-local motion encoder with a hierarchical attention pooling block and a GRU-based decoder to extract motion details from the sparse-view references, which takes the concatenated $\mathcal{Q}$ and $\mathcal{C}$ as input.
%
In our encoder, we design two branches to encode the global and local skeletal motion features independently.
%
Note that we mainly use 1D convolution layers during the encoding process to extract corresponding temporal information.
% 
We apply three layers of 1D convolution for the global branch while splitting the input motion map into $N_J$ local quaternions for the local branch inspired by \cite{taew}.
%
Differently, we utilize a hierarchy attention pooling layer to connect the feature of adjacent joints and compute the latent codes from five local body regions, including the four limbs and the torso.
%
We concatenate the global and local feature of two branches as the final latent code, and decode them to the original quaternions domain with three linear layers in our GRU-based decoder (see Fig.~\ref{fig:fig_3_network} for detail).
%
Here, the loss of our generator $\mathcal{G}$ is formulated as:
\begin{align}
\mathcal{L}_{\mathcal{G}} = \mathcal{L}_{sv} + \mathcal{L}_{adv},
\end{align}
where $\mathcal{L}_{sv}$ is the sparse-view loss and $\mathcal{L}_{adv}$ is the adversarial loss.
%
Our sparse-view loss is formulated as:
\begin{align}
& \mathcal{L}_{sv} = \sum_{t=1}^T \left\|\hat{\textbf{Q}}_t - \textbf{Q}^{sv}_t\right\|_2^2 + \lambda_{quat}\sum_{t=1}^T\sum^{N_J}_{i=1}(\|\hat{\textbf{Q}}_t^{(i)}\| - 1)^2.
\end{align}
%
Here, the first term is the $L_2$ loss between the regressed output motion $\hat{\textbf{Q}}_t$ and the 3D motion prior $\textbf{Q}^{sv}_t$ from sparse-views reference.
%
Note that we obtain $\textbf{Q}^{sv}_t$ from the reference sparse multi-view images by directly extending the same optimization process to the multi-view setting.
%
The second regular term forces the network output quaternions to represent a rotation.
%
Besides, $N_J$ denotes the number of joints which is 15 in our case while $\lambda_{quat}$ is set to be $1\times 10^{-5}$.


% 2. marker-based reference
Our motion discriminator $\mathcal{D}$ further utilizes the motion characteristics from the unpaired marker-based references, which maps the motion map $\mathcal{\hat{Q}}$ corrected by the generator to a value $\in [0, 1]$ to represent the probability $\mathcal{\hat{Q}}$ is a plausible human challenging motion.
%
Specifically, we follow the video motion capture approach VIBE~\cite{VIBE_CVPR2020} to design two losses, including the adversarial loss $\mathcal{L}_{adv}$ to backpropagate to the generator $\mathcal{G}$ and the discriminator loss $\mathcal{L}_{\mathcal{D}}$ for the discriminator $\mathcal{D}$:
\begin{align}
    &\mathcal{L}_{adv} = \mathbb{E}_{\mathcal{\hat{Q}} \sim p_{\mathcal{G}}}\left[\left(\mathcal{D}(\mathcal{\hat{Q}})-1\right)^{2}\right],\\
	&\mathcal{L}_{\mathcal{D}} = \mathbb{E}_{\mathcal{Q}^{mb} \sim p_{V}}\left[\left(\mathcal{D}(\mathcal{Q}^{mb})-1\right)^{2}\right]+\mathbb{E}_{\mathcal{\hat{Q}} \sim p_{\mathcal{G}}}\left[\left(\mathcal{D}(\mathcal{\hat{Q}})\right)^{2}\right].
\end{align}
%
Here, the adversarial loss $\mathcal{L}_{adv}$ is the expectation that $\mathcal{\hat{Q}}$ belongs to a plausible human challenging motion, while $p_{\mathcal{G}}$ and $p_V$ represents the corrected motion sequence the corresponding captured maker-based challenging motion sequence, respectively.
%
Note that $\mathcal{Q}^{mb}$ denotes the accurate but temporally unsynchronized motion map captured by the marker-based system.
%
Compared to VIBE~\cite{VIBE_CVPR2020} which extracts general motion prior, our scheme can recover the characteristics of more specific challenging motion.



\myparagraph{Training Details.}
We train our HybridNet for 500 epochs with Adam optimizer~\cite{kingma2014adam}, and set the dropout ratio as 0.1 for the GRU layers.
%
We apply Exponential Linear Unit (ELU) activation and batch normalization layer after every our 1D convolutional layer with kernel size 7, except the final output layer before the decoder.
%
During training, four NVidia 2080Ti GPUs are utilized.
%
The batch size is set to be 32, while the learning rate is set to be $1 \times 10^{-3}$ for the generator and $1 \times 10^{-2}$ for the discriminator, the decay rate is 0.1 (final 100 epochs).
%
To train our HybridNet, a new dataset with rich references modalities and various challenging motions and performers is further introduced and more details about our dataset are provided in Sec.~\ref{ExperimentalResults}

%
Our hybrid motion inference utilizes multi-modal references to extract fine motion details for challenging human motions in a data-driven manner.
%
At test time, our method can robustly boost the tracking accuracy of the initial noisy skeletal motions via a novel generation network.
%
Since our learning scheme is not directly supervised on the input images of specific performers, it's not restricted by per-performer training.
%
Instead, our approach focus on extracting the characteristics of challenging motions directly.


%% --------------------------------------------------------------
%% --------------------------------------------------------------




\begin{figure*}
	\centering
	\includegraphics[width=0.95\linewidth]{figures/rs_gallery.pdf}
	\caption{3D capturing results on challenging human motions. For each body motions, the top row shows the input images, the middle row shows the captured body results on camera view, and the bottom row shows the rendering result of the captured body from side view. }
	\label{fig:rs_gallery}
\end{figure*}


==> cache/M_2.tex <==
\subsection{Robust Motion Optimization}
\label{sec:mot_optimization}
Besides the data-driven 3D motion characteristics from the previous stage, the input RGB video also encodes reliable motion hints for those non-extreme poses, especially for the non-occluded regions. We thus introduce this robust motion optimization to refine the skeletal motions so as to increase the tracking accuracy and overlay performance, which jointly utilizes the learned 3D prior from the supervised multi-modal references as well as the reliable 2D and silhouette information from the input image references.
%
The optimization to refine the skeletal pose is formulated as:
\begin{align} \label{eq:opt}
\boldsymbol{E}_{\mathrm{total}}(\textbf{S}_t) = \boldsymbol{E}_{\mathrm{3D}} + \lambda_{\mathrm{2D}}\boldsymbol{E}_{\mathrm{2D}} + \lambda_{\mathrm{T}}\boldsymbol{E}_{\mathrm{T}} + \lambda_{\mathrm{S}}\boldsymbol{E}_{\mathrm{S}}.
\end{align}
Here, $\boldsymbol{E}_{\mathrm{3D}}$ makes the final motion sequence close to the output of network on occluded and invisible joints while  $\boldsymbol{E}_{\mathrm{2D}}$ adds a re-projection constraint on high-confidence 2D keypoints detected. $\boldsymbol{E}_{\mathrm{T}}$ enforces the final motion to be temporally smooth, while the $\boldsymbol{E}_{\mathrm{S}}$ enforces alignment of the projected 3D model boundary with the detected silhouette.
% Furthermore, the optimization process takes hip global translation into consideration compared to the network.
%
Specifically, the 3D term $\boldsymbol{E}_{\mathrm{3D}}$ is as following:
\begin{align}
\boldsymbol{E}_{\mathrm{3D}} = \sum^T_{t=1}\|\textbf{S}_t - \mathcal{M}(\hat{\textbf{Q}}_t,\textbf{t}_t)  \|^2_2,
\end{align}
where $\hat{\textbf{Q}}_t$ is the regressed quaternions motion from our previous stage; $\mathcal{M}$ is the mapping from quaternions to skeletal poses; $\textbf{t}_t$ is the global translation of $\textbf{S}_t$.
%
Note that the joint angles $\boldsymbol{\theta}_t$ of $\textbf{S}_t$ locate in the pre-defined range $[\boldsymbol{\theta}_{min},  \boldsymbol{\theta}_{max}]$ of physically plausible joint angles to prevent unnatural poses.
%
We then propose the projected 2D term as:
\begin{align}
\boldsymbol{E}_{\mathrm{2D}} = \frac{1}{T}\sum^T_{t=1}\frac{1}{|C_t|}\sum_{i\in C_t
}\|\Pi(J_i(\textbf{S}_t))-\mathbf{p}_{t}^{(i)}\|^2_2,
\end{align}
where $C_t = \{ i \ |\  c_t^{(i)} \geq thred \}$ is the set of indexes of high-confidence keypoints on the image $I_t$; $ c_t^{(i)}$ is the confidence value of the $i^{th}$ keypoint $\mathbf{p}_{t}^{(i)}$; $thred$ is 0.8 in our implementation. 
%
The projection function $\Pi$ maps 3D joint positions to 2D coordinates while $J_i$ computes the 3D position of the $i^{th}$ joint. 
%
Then, the temporal term $\boldsymbol{E}_{\mathrm{T}}$ is formulated as:
\begin{align}
\boldsymbol{E}_{\mathrm{T}} = \sum^{T-1}_{t=1}\|\mathcal{M}(\hat{\textbf{Q}}_t,\textbf{t}_t) - \mathcal{M}(\hat{\textbf{Q}}_{t+1},\textbf{t}_{t+1})\|^2_2,
\end{align}
where $\hat{\textbf{Q}}_t$ and $\hat{\textbf{Q}}_{t+1}$ are two adjacent regressed quaternions motion from our hybrid motion inference module. 
%
We utilize temporal smoothing to enable globally consistent capture in 3D space.
%
Moreover, we follow \cite{MonoPerfCap} to formulate the silhouette term $\boldsymbol{E}_{\mathrm{S}}$ and please refer to \cite{MonoPerfCap} for more detail.


% Optimization
The constrained optimization problem to minimize the Eqn.~\ref{eq:opt} is solved using the Levenberg-Marquardt (LM) algorithm of  
\textit{ceres}~\cite{ceresSolver}.
%
In all experiments, we use the following empirically determined parameters: $\lambda_{\mathrm{2D}} = 1.0$, $\lambda_{\mathrm{T}} = 20.0$ and $\lambda_{\mathrm{S}} = 0.3$.
%
Note that the initial $\textbf{t}_t$ for the mapping from quaternions to skeletal poses is obtained through the pre-processing stage in Sec.~\ref{sec:mot_inference}.
%
To enable more robust optimization, we first optimize the global translation $\textbf{t}_t$ for all the frames and then optimize the $\textbf{S}_t$.
%
Such a flip-flop optimization strategy improves the overlay performance and tracking accuracy, which jointly utilizes the 3D challenging motion characteristics from the supervised multi-modal references as well as the reliable 2D and silhouette information from the input image references.







==> cache/Method_backup.tex <==
% ps1: 网络的attention pooling操作借鉴了take an emotion walk paper https://arxiv.org/pdf/1911.08708.pdf
% 在其上做的主要改进为 1. 加入confidence prior 2. 结合global和local的信息 详见下面和框图
% ps2: 网络用到的主要operation 为conv1d 和 batchnorm1d 激活函数为ELU
% ps3: 目前其实没有用到vicon的reference 是纯用multiview伪GT来做监督的 vicon这一部分怎么往里加还需要考虑 我近期也会真的考虑加到网络里 (要么和第1部分的motion map一起过网络 要么后接一个discriminator 后者工作量和训练时间都会大幅加大

% 输入 motion map & confidence map
% 输出 refined motion map (T, 35)

% sparse view GT 获取方式. 用4个view的信息做和第1步流程一致的IK 优化的cost function里 叠加4个view的reprojection loss即可
% mocap data: 通过vicon系统拍摄 时序与rgb video不align

% i. 将输入的两种map都整理成quaterion形式 size都变成了(T, 13*4) 两种map做元素乘得到fused map (T, 52)

% ii. 过网络 网络分为两个主要的branch 一个提取global信息 使用了2层conv1d 另一个分支提取人体各个不同part的local信息 这一部分详见iii
% iii. 提取local信息 首先按照不同joint的语义把输入的motion map划分为13个(T, 4) 将它们分别过conv1d之后得到13个(T, 96) 然后把临近的身体部位加权求和
% (eg: left_down = 0.4 * left_hip + 0.4 * left_knee + 0.2 * left_ankle
%     left_up = 0.4 * left_sho + 0.4 * left_elb + 0.2 * left_clv) 这个操作叫做attention pooling 借鉴take an emotion walk paper https://arxiv.org/pdf/1911.08708.pdf page8 fig.2
% iv. 最终得到5种local information 将它们再过一系列conv1d后 和第1个branch得到的global feature concat到一起 再过mlp和gru decode出output motion map (详见框图)


% (MonoPerfCap: Our 2D joint alignment term is a re-projection constraint enforcing that the projected joint positions $J_i(S_f)$ closely match the corresponding 2D detections) % J_i is essentially a forward kinematic process
%(MonoPerfCap: where the hard constraints on the per-frame joint angles Θf are physically motivated and ensure the reconstruction of plausible
% human body poses by forcing the joint angles to stay inside their anatomical lower Θmin and upper Θmax bounds [Stoll et al. 2011].)















%To generate the initial 3D motions, we first utilize an effective inverse kinematics optimization \cite{MonoPerfCap} with estimated 2D poses from OpenPose \cite{openpose}. Then, we propose a joint optimization with 2D/3D term to estimate the final 3D motion sequences.

%\he{For initial rough 3D motions, we first rig the corresponding template model $S$ with skeleton of 36 degrees of freedom (DOFs), and estimate the heat map $xx$ of 2D keypoints with 2D pose detector~\cite{openpose}. 
%We utilize an effective inverse kinematics optimization from \cite{MonoPerfCap}
%\begin{align}
%	E_{init} = \frac{1}{T}\sum^T_{t=1}\frac{1}{N_P}\sum^{N_P}_{i=1}\|\Pi(J_i(\mathcal{M}(\hat{\mathbf{Q}}^{init}_t)))-p_{t}^{(i)}\|^2_2 
%\end{align}
%where $\mathcal{M}(\hat{\mathbf{Q}}^{init}_t) \in \mathbb{R}^{36}$ located in $[\Theta_{min}, \mathbf{\Theta}_{max}]$, $\mathcal{M}$ is the function mapping quaternions to axis-angles. We choose axis-angle form representation since we can We can add constraints on human joints with different number of dimensions according to the inherent structure of the human body, and set numerical boundaries for different dimensions of body joints. \cite{stoll2011fast}
%$N_P$ is the number of 2D keypoints, $p_{t}^{(i)}$ is the $i^{th}$ keypoint coordinate in $I_t$. $\Pi$ is the mapping $\mathbb{R}^3 \rightarrow \mathbb{R}^2$ with full perspective projection, $J_i$ transfer axis angle $\mathbf{\Theta}_t$ to the $i^{th}$ 3D joint location.
%Since we limit dimension numbers on different body joints, for balancing the contribution of joints, we transfer the axis-angles to quaternions \cite{pavllo2018quaternet} $\mathbf{Q}^{init} \in \mathbb{R}^{T\times 4N_J}$ , then pass it into the hybrid motion inference network above. $N_J$ is total joint number. 




















==> cache/Overview.tex <==
% 说明文章的研究目标 - monocular 3D human motion capture for challenging poses.
% 问题的难点 单目的歧义性 身体的自遮挡 连续运动容易出现抖动 和 不稳定
% 为此 我们提出xxx的数据集xx包含spart view xxx pose,  以及动作内容相同的3D motion capture data from marked suit and multi-view MoCap system (Vicon)
% 我们的方法总述：构建xxx module，同时利用sparse-view 对齐但不一定合理的数据 和 动作准确合理但不一定对齐的数据，然后 xxx的优化
%In this paper, we tackle the above challenges and present \textit{ChallenCap} -- a template-based monocular 3D  capture approach for challenging human motions from a single RGB video, which outperforms existing state-of-the-art approaches significantly (See Fig.~\ref{fig:fig_1_teaser} for an overview). Our novel pipeline proves the effectiveness of embracing multi-modal references from both temporally unsynchronized marker-based system and light-weight markerless multi-view system in a data-driven manner, which enables robust human motion capture under challenging scenarios with extreme poses and complex motion patterns, whilst still maintaining monocular setup.
% 1 intro methods
%our ChallenCap utilizes a hybrid motion module learned with a weakly supervision from sparse-view estimated poses and the relevant MoCap data, and build an effective optimization with the priors of 2D/3D poses for accurate and reliable 3D poses,
% 2. Dataset
% To model this challenging motion capture problem in a data-driven manner, we collect a new Sparse-view Challenging Motion Capture (SCMC) dataset, which contains both video clips from four views as well as the corresponding relevant 3D motions captured via a motion capture system.

\section{Overview}
Our goal is to capture challenging 3D human motions from a single RGB video, which suffers from extreme poses, complex motion patterns and severe self-occlusion.
%
Fig.~\ref{fig:overview} provides an overview of ChallenCap, which relies on a template mesh of the actor and makes full usage of multi-modal references in a learning-and-optimization framework.
%
Our method consists of a hybrid motion inference module to learn the challenging motion characteristics from the supervised references modalities, and a robust motion optimization module to further extract the reliable motion hints in the input images for more accurate tracking.
% A brief introduction of our main components is provided as follows.

\myparagraph{Template and Motion Representation.}
We use a 3D body scanner to generate the template mesh of the actor and rig it by fitting the Skinned Multi-Person Linear Model (SMPL)\cite{SMPL2015} to the template mesh and transferring the SMPL skinning weights to our scanned mesh.
%
The kinematic skeleton is parameterized as $\textbf{S}=[\boldsymbol{\theta}, \textbf{R},\textbf{t}]$, including the joint angles $\boldsymbol{\theta} \in \mathbb{R}^{30}$ of the $N_J$ joints, the global rotation $ \textbf{R}\in\mathbb{R}^3$ and translation $\textbf{t} \in \mathbb{R}^{3}$ of the root.
%
Furthermore, let $\textbf{Q}$ denotes the quaternions representation of the skeleton.
%
Thus, we can formulate $\textbf{S}=\mathcal{M}(\textbf{Q},\textbf{t})$ where $\mathcal{M}$ denotes the motion transformation between various representations.

% During motion inference, we design a novel network architecture, HybridNet, supervised via the references from both the unsynchronized marker-based and sparse multi-image systems. Note that the former marker-based reference encodes the accurate spatial motion characteristics but sacrifices the temporal consistency, while the latter multi-image reference provides overall 3D motion priors but fails to capture extreme poses.
% To avoid per-performer training and encode temporal motion information, we first obtain the initial noisy skeletal motion from monocular video as the input to our HybridNet.  
% Then, a novel loss or network XXXX


% 1. initial noisy skeletal motions --> quaternions motion map
% 2. GAN; encoder, decoder; multi-modal refernces
%  Temporal Encoder; Motion Discriminator
% 3. Dataset
\myparagraph{Hybrid Motion Inference.}
Our novel motion inference scheme extracts the challenging motion characteristics from the supervised marker-based and sparse multi-view references in a data-driven manner.
%
We first obtain the initial noisy skeletal motion map from the monocular video.
%
Then, a novel generation network, HybridNet, is adopted to boost the initial motion map, which consists of a temporal encoder-decoder to extract local and global motion details from the sparse-view references, as well as a motion discriminator to utilize the motion characteristics from the unpaired marker-based references.
%
To train our HybridNet, a new dataset with rich references modalities and various challenging motions is introduced (Sec. \ref{sec:mot_inference}).

% To tackle the monocular ambiguity and self-occlusion, we propose the hybrid motion module to model the feasible real world human poses for challenging video input via attention-based xxx network structure. Based on the prior of such hybrid motion poses, we further introduce this novel network to estimate the feasible poses from rough input so as to recover the reliable 3D motions. Our hybrid motion module consists of a attention-based xxx encoder, a xxx decoder to regress the poses from both global and local xxx (features), xxx to the 3D motion output . For weakly supervision, we formulate the xxx loss, the xxx loss, to train this hybrid motion net with the xx ability.


\myparagraph{Robust Motion Optimization.}
Besides the data-driven 3D motion characteristics from the previous stage, the input RGB video also encodes
reliable motion hints for those non-extreme poses, especially for the non-occluded regions.
%
Thus, a robust motion optimization is introduced to refine the skeletal motions so as to increase the tracking accuracy and overlay performance, which jointly utilizes the learned 3D prior from the supervised multi-modal references as well as the reliable 2D and silhouette information from the input image references (Sec. \ref{sec:mot_optimization}).

% For a challenging video input, we utilize the mentioned hybrid motion net to formulate an effective spatio-temporal optimization on the pose sequences. Based on a simple 3D pose estimator to produce the rough 3D poses input, We further propose this batch-based optimization, including xxx term and xxx, which enables stable and reliable 3D pose sequences for challenging motion captured with monocular camera.

% The following sections provide the details of the full system.



==> cache/Related.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig_2_overview}
	\caption{The pipeline of ChallenCap with multi-modal references. Assuming the video input from monocular camera, our approach consists of a hybrid motion inference stage (Sec.\ref{sec:mot_inference}) and a robust motion optimization stage (Sec.\ref{sec:mot_optimization}) to capture 3D challenging motions. $\mathcal{D}$ represents the discriminator. }  %\textcolor{red}{[Ma: Could we have descriptions or fill in content for the vacant boxes and trapezoid? In addition, give more description in the caption.]}
	\label{fig:overview}
\end{figure*}


\section{Related Work}
As an alternative to the widely used marker-based solutions~\cite{VICON,Xsens,Vlasic2007}, markerless motion capture~\cite{BreglM1998,AguiaSTAST2008,TheobASST2010} technologies alleviate the need for body-worn markers and have been widely investigated.
%
In the following, we focus on the field of marker-less 3D human motion capture.

\myparagraph{Parametric Model-based Capture.}
Many general human parametric models~\cite{SCAPE2005,SMPL2015,SMPLX2019,STAR_ECCV2020} learned from thousands of high-quality 3D scans have been proposed in the last decades, which factorize human deformation into pose and shape components. 
% human shape prior by using human parametric models 
Deep learning is widely used to obtain skeletal pose and human shape prior through model fitting~\cite{TAM_3DV2017,Lassner17,keepitSMPL,Kolotouros_2019_CVPR} or directly regressing the model parameters from the input~\cite{HMR18,Kanazawa_2019CVPR,VIBE_CVPR2020,zanfir2020neural}.
%
Besides, various approaches~\cite{detailHuman_2019CVPR,DetailDepth_2019ICCV,People3D_2019ICCV,TEX2SHAPE_2019ICCV,DeepHuman_2019ICCV} propose to predict detailed human geometry by utilizing parametric human model as a basic estimation.
%
Beyond human shape and pose, recent approaches further include facial and hand models~\cite{Xiang_2019_CVPR,TotalCapture,SMPLX2019,MonoExpressive_ECCV2020} for expressive reconstruction or leverage garment and clothes modeling on top of parametric human model~\cite{ClothCap,bhatnagar2019mgn,TailorNet_CVPR2020,LearnToDress_CVPR2020}.
%
But these methods are still limited to the parametric model and cannot provide space-time coherent results for loose clothes. 
%
Instead, our method is based on person-specific templates and focuses on capturing space-time coherent challenging human motions using multi-modal references.



\myparagraph{Free-form Volumetric Capture.}
% fusion-based method
Free-form volumetric capture approaches with real-time performance have been proposed by combining the volumetric fusion \cite{Curless1996} and the nonrigid tracking~\cite{sumner2007embedded,li2009robust,zollhofer2014real,guo2015robust} using depth sensors. 
%
The high-end solutions~\cite{dou-siggraph2016,motion2fusion,UnstructureLan,TheRelightables} rely on multi-view studios which are difficult to be deployed.
%
The most handy monocular approaches for general non-rigid scenes~\cite{Newcombe2015,innmann2016volume,guo2017real,KillingFusion2017cvpr,slavcheva2018cvpr,slavcheva2020pami,FlyFusion} 
can only capture small, controlled, and slow motions.
%
Researchers further utilize parametric model~\cite{BodyFusion,DoubleFusion,UnstructureLan,robustfusion} or extra body-worn sensors~\cite{HybridFusion} into the fusion pipeline to increase the tracking robustness.
%
However, these fusion approaches rely on depth cameras which are not as cheap and ubiquitous as color cameras.
% data-driven metthods
Recently, the learning-based techniques enable free-form human reconstruction from monocular RGB input with various representations, such as volume~\cite{DeepHuman_2019ICCV}, silhouette~\cite{SiCloPe_CVPR2019} or implicit representation~\cite{PIFU_2019ICCV,PIFuHD,MonoPort,Chibane_2020CVPR,Implicit_ECCV2020}.
%
However, such data-driven approaches do not recover temporal-coherent reconstruction, especially under the challenging motion setting. 
%
In contrast, our template-based approach can explicitly obtain the per-vertex correspondences over time even for challenging motions.

\myparagraph{Template-based Capture.}
A good compromising settlement between from-form capture and parametric Modal-based Capture is to utilize a specific human template mesh as prior.
%
Early solutions~\cite{Gall2010,StollHGST2011,liu2013markerless,Robertini:2016,Pavlakos17,Simon17,FlyCap} require multi-view capture to produce high quality skeletal and surface motions but synchronizing and calibrating multi-camera systems is still cumbersome. 
%
Recent work only relies on a single-view setup~\cite{MonoPerfCap,LiveCap2019tog,EventCap_CVPR2020} achieve space-time coherent capture and even achieves real-time performance~\cite{LiveCap2019tog}.
%
However, these approaches fail to capture the challenging motions such as yoga or rolling on the floor, which suffer from extreme poses and severe self-occlusion under the monocular setting. 
%
The recent work~\cite{DeepCap_CVPR2020} utilizes weekly supervision on multi-view images directly so as to improve the 3D tracking accuracy during test time.
%
However, their training strategy leads to dedicated per-performer training.
%
Similarly, our approach also employs a person-specific template mesh.
%
Differently, we adopt a specific learning-and-optimization framework for challenging human motion capture.
%
Our learning module is supervised on the motion itself instead of the input images of specific performers for improving the generation performance to various performers and challenging motions. 
%\textcolor{red}{[Ma: How could we achieve the generalization for various performers? Do we explain it in other parts?]}


\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/fig_3_network}
	\caption{Illustration of our hybrid motion network,  HybridNet, which encodes the global and local temporal motion information with the losses on both the generator and the discriminator. Note that the attention pooling operation is performed by applying element-wise addition (blue branches) on the features of the adjacent body joints. The features after attention pooling are concatenated together with the global feature as input to the fully connected layers.}
	%\textcolor{red}{[Ma: Could we mark the encoder and decoder areas and the discriminator to make the structure clearer? $L_{mc}$ loss equals to $L_{D}$? It is better to unify the representation or give explanation. In addition, give more description in the caption.]}
	\label{fig:fig_3_network}
\end{figure*}


==> cache/conclusion.tex <==
\section{Discussion}
\myparagraph{Limitation.}
As the first trial to explore challenging human motion capture with multi-modal references, the proposed ChallenCap still owns limitations as follows.
% 1. template
First, our method relies on a pre-scanned template and cannot handle topological changes like clothes removal.
% 2. object interaction scenes with severe human-object occlusion
Our method is also restricted to human reconstruction, without modeling human-object interactions.
%
It's interesting to model the human-object scenarios in a physically plausible way to capture more challenging and complicated motions.
% 3. in an end-to-end manner
Besides, our current pipeline turns to utilize the references in a two-stage manner.
%
It’s a promising direction to formulate the challenging motion capture problem in an end-to-end learning-based framework.

\myparagraph{Conclusion.}
We present a robust template-based approach to capture challenging 3D human motions using only a single RGB camera, which is in a novel two-stage learning-and-optimization framework to make full usage of multi-modal references.
%
Our hybrid motion inference learns the challenging motion details from various supervised references modalities, while our robust motion optimization further improves the tracking accuracy by extracting the reliable motion hints in the input image reference.
%
Our experimental results demonstrate the effectiveness and robustness of ChallenCap in capturing challenging human motions in various scenarios.
%
We believe that it is a significant step to enable robust 3D capture of challenging human motions,
with many potential applications in VR/AR, and performance evaluation for gymnastics, sports, and dancing.

% which compares favorably to the state-of-the-arts.
%it suffers from complex motion patterns and severe self-occlusion under the monocular setting. 






==> my_section/Intro.tex <==
\section{Introduction}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\linewidth]{fig/teaser.pdf}
	\caption{The two-stage models vs our proposed one-stage Vote2Cap-DETR}
	\label{fig:teaser}
\end{figure}


% 1. Dense-Captioning on 3D scenes is important
3D dense captioning \ct{give several refers} requires to localize all the objects in a 3D scene, and generate descriptive sentences for each object, which can benefit many applications such as natural language control in VR/AR systems and home appliance intelligence， and has raised great interest among scholars in recent years~\cite{chen2021scan2cap,chen2021d3net,yuan2022x-trans2cap,wang2022spacap3d,jiao2022more,cai20223djcg}.

% our understanding of this task and issues
\textcolor{red}{The key to the 3D dense captioning problem is \textbf{accurate localization} of all potential objects in a 3D scene as well as \textbf{informative description generation}.}
%
% Different categories of works
%
% First class: relation modelling specified
%
Scan2Cap\cite{chen2021scan2cap}, MORE\cite{jiao2022more}, and SpaCap3D\cite{wang2022spacap3d} propose well-designed relation reasoning modules to efficiently model relations among object proposals.
%
% Second class: joint training of grounding and captioning
%
3DJCG\cite{cai20223djcg} and D3Net\cite{chen2021d3net} study the correlation between 3D visual grounding and 3D dense captioning and point out that these two task promote each other.
%
% Third class: 2D to 3D knowledge transfer
%
Additionally, $\chi$-Trans2Cap\cite{yuan2022x-trans2cap} analyzes how to transfer knowledge from additional 2d information to boost 3d dense captioning.
%
% Issue of these existing works
%
Though all the above methods have achieved great results, they all follow a detect-then-describe pipeline which suffers from the following issues:
%
%\textbf{exploiting reasoning object proposals' relationship}
(1) The scene contextual information such as the background is overlooked when reasoning relationships among object proposals, causing accumulated errors from the detector output. 
%error from the detector output may be accumulated directly reasoning relationships among object box predictions accumulates error from the detector, overlooks implicit contextual information such as the background;
%
(2) The learning of object detection and captioning process is not well connected and unified, i.e. the captioner under-utilizes the feature produced by the detector, and the detector does not benefit from the captioning process.
% (2) Proposal level interaction fails to complement each object with elements a detector overlooks or can not perceive.
%
(3) The traditional one-to-one training strategy optimizes one single sentence generation for each scene, leading to slow convergence of the captioner training due to that there usually exist multiple labelled sentences for one scene.
% (3) The feature produced by the object detector fails to capture abundant attribute or surrounding information to guide the captioner.
%
% additional issues with 3DETR
Recently, DETR\cite{carion2020detr}, a encoder-decoder architecture has a great success in various computer vision tasks.
%
In 3D object detection, 3DETR\cite{misra2021-3detr} achieves promising performance with a pure transformer based model, which also suits 3D dense captioning.
%
However, it suffers from huge memory cost and slow convergence.

% We 将要，致力于 处理这些问题..
To address the above issues, we propose Scene2Cap, an encoder-decoder transformer based system for 3D dense captioning, which detect objects with \textcolor{red}{global scene information} and describe object with both \textcolor{red}{local scene information}.
% To address the above issues, \cx{we propose Scene2Cap, a context-aware transformer based system, which leverages local \textcolor{red}{information} and global \textcolor{red}{scene information} for \textcolor{red}{accurate} 3D dense captioning.}
%
Because of the high memory cost and slow convergence problem of 3DETR\cite{misra2021-3detr}, we replace the scene encoder to PointNet++\cite{qi2017pointnet++}.
%
Following the scene encoder is an object decoder for object detection, and another decoder for caption generation.
%
%
% Object Decoder
%
%
To deal with the slow convergence problem, we propose novel vote queries as initial object queries to accelerate training and boost the detection performance.
%
Thanks to object decoder's built-in self-attention for proposal-proposal interaction and cross-attention for implicit scene information complementing, we can efficiently model relationship and fuse information for each proposal.
%
%
% Caption Decoder
%
%
To generate informative descriptions for each object, our caption decoder receives visual clue by two means.
%
We concatenate object proposals with caption queries to keep the caption decoder inform the object to be described.
%
Then, we complement the caption decoder with scene tokens nearby a proposal via cross-attention to inform a surrounding surrounding information, which is less sensitive to the detector's output than the traditional k nearest valid box proposal\cite{chen2021scan2cap,cai20223djcg,chen2021d3net}.
%
We further use an additive learnable embedding to identify whether a scene token belongs to the object, which help generate more informative caption.
%
To this end, our caption decoder 
%

% intro your xx detector and xx captioner
% Scene2Cap contains an object detector with built-in proposal level interactions, and a captioner.
% Scene2Cap contains an object detector with built-in proposal level interactions, and a natural language generator.
%
% The Detector
% Specifically, the \cx{describe-its} detector first extract features for the input pointcloud with a Pointnet++ backbone\cite{qi2017pointnet++}, and generate box queries with the voting module from \cite{qi2019votenet} and a set abstraction layer from \cite{qi2017pointnet++}.
%
% The Captioner.
% Meanwhile, the \cx{describe-its} captioner \cx{tell-it-function}is a masked transformer decoder based model.
% Meanwhile, the \cx{describe-its} captioner \cx{tell-it-function} first xx.
% cx:then 
% We extend the proposal feature to the caption prefix to inform the captioner the object to be described as \cite{wang2022spacap3d}.
% cx:connection between detector and captioner
% Besides, we introduce local context feature from a proposal's surroundings through cross-attention, which complements the language generation procecss with attribute information and surrounding information.

% Supervision
Different from existing works, we formulate 3D dense caption as a set-to-set prediction problem inspired by \cite{carion2020detr,misra2021-3detr}.
During training, we match each annotated object with one unique proposal, and supervise their caption generation process.
Our training strategy preserves the data distribution of the detection dataset and further boosts the convergence speed of the full model.
Additionally, our method can achieve a better balance between detection and captioning.
To this end, we further narrow the gap between training and evaluation.

\textbf{Contributions}. Our contributions include:
\begin{itemize} 
\setlength\itemsep{0em}
    \item We propose a novel contextual information driven approach for 3D dense captioning, which contains a detector with built-in proposal level interactions and a contextual aware captioner.
	To our knowledge, this is the first attempt analyzing how contextual information benefits 3D dense captioning.
	
	\item We formulate the 3D dense captioning problem as a set-to-set prediction problem, which achieves a better balance between detection and captioning and narrows the gap between training and evaluation.

	\item Extensive experiments show that our proposed Scene2Cap approach achieves a new state-of-the-art performance on both Nr3D\cite{achlioptas2020referit3d}(-\% C@0.5) and ScanRefer\cite{chen2021scan2cap}(-\% C@0.5).
	
\end{itemize} 


==> my_section/IntroV2.tex <==
\section{Introduction}

% paragragh 1. Dense-Captioning on 3D scenes is important
3D dense captioning \cite{chen2021scan2cap,chen2021d3net,yuan2022x-trans2cap,wang2022spacap3d,jiao2022more,cai20223djcg} requires a system to localize all the objects in a 3D scene, and generate descriptive sentences for each object. 
%
Combining scene understanding with natural language generation, researches on 3D dense captioning benefit many applications such as natural language control in VR/AR systems and home appliance intelligence. 
%
This problem is challenging given 1) the sparsity and occlusions of point clouds and 2) the cluttered and unbalanced distribution of object-caption pairs. 
%
\csj{sparsity \& occlusion may not be solved in this paper?}

% paragragh 2. our understanding of this task and issues
% \textcolor{red}{The key to the 3D dense captioning problem is \textbf{accurate localization} of all potential objects in a 3D scene as well as \textbf{informative description generation}. 
Existing methods follows a "one two three" pipeline by first producing object proposals, then modelling object relations, and finally performing description of object regions. 
%
Most existing works focus a few aspects of the pipeline. 
%
Scan2Cap\cite{chen2021scan2cap}, MORE\cite{jiao2022more}, and SpaCap3D\cite{wang2022spacap3d} propose well-designed relation reasoning modules to efficiently model relations among object proposals.
%
% Second class: joint training of grounding and captioning
%
3DJCG\cite{cai20223djcg} and D3Net\cite{chen2021d3net} study the correlation between 3D visual grounding and 3D dense captioning and point out that these two task promote each other.
%
% Third class: 2D to 3D knowledge transfer
%
Additionally, $\chi$-Trans2Cap\cite{yuan2022x-trans2cap} analyzes how to transfer knowledge from additional 2d information to boost 3d dense captioning.

On the other hand, most of these methods relies on many hand-crafted components and learning strategies.e.g radii and designing 3D operators and loss function to produce satisfactory localization and description. 
%
Firstly, most existing methods rely on VoteNet detector for object proposals, which will produce many overlapped boxes with non-maximal suppression and leads to slow feature extraction and fluctuate caption efficiencies.
%
\csj{which produce overlapping boxes and confuse the relationship reasoning, and its heavy dependence on non-maximal suppression leads to poor efficiency.}
%
Secondly, the implicit scene contextual information is overlooked when reasoning relationships among explict object proposals, which leads to lower captioning performance.
%
\csj{leading to limited environmental awareness and lower captioning performance.}
%
Thirdly, existing methods need to exhaustive train the whole dataset's sentences, which leads unstabilitye \csj{unstabilized} training of the captioning module and overfit to the scenes with many object-caption pairs.

Inspired by recent 3D DEtection TRansformer
(3DETR)\csj{\cite{misra2021-3detr}} that uses fewer hand-coded design decisions with fully attentional design and also casts detection as a set-to-set problem, our work explore an fully transformer encoder-decoder architecture to resolve the curse of 3D dense captioning with following three innovations: 
%
1) Our method consider the 3D dense captioning task as a set prediction problem. The proposed Vote2Cap-DETR directly decodes the features into an object sets with their locations and corresponding captions by applying two parallel prediction heads. 
%
2) we propose a novel vote decoder by reformulate the object queries in 3DETR into the format of the vote query that is a composition of the embeddings of the seeds point and the vote transformation of the box with respect to the seeds, which indicates the connection between the vote query in Vote2CAP-DETR with the VoteNet, but with better localization and higher training efficiencies; 
%
3) we develop a novel caption query driven head, which absorbs the relation and attribute modelling into the self- and cross-attnetion such that it can looks into both the local and global scene context to better describe.
%
Extensive experiments on two commonly used datasets, ScanRefer and Nr3D, demonstrate that our approach can achieve can surpass SOTA with many hand-craft procedures with large margin \csj{by large margin}, which demonstrates the supriority of that fully transformer architecture with sophisticated vote head and caption head can inspire many 3D vision and language tasks. 

To summarize, the main contribution of this work include:
\begin{itemize} 
\setlength\itemsep{0em}
    \item We propose a novel one-stage and fully attention driven architecture for 3D dense captioning as a set-to-set prediction problem, which achieves a better balance between detection and captioning and narrows the gap between training and evaluation.

	\item Extensive experiments show that our proposed Vote2Cap approach achieves a new state-of-the-art performance on both Nr3D\cite{achlioptas2020referit3d}(-\% C@0.5) and ScanRefer\cite{chen2021scan2cap}(-\% C@0.5).
	
\end{itemize} 







% } 
%


==> my_section/Overview.tex <==
% 说明文章的研究目标 - monocular 3D human motion capture for challenging poses.
% 问题的难点 单目的歧义性 身体的自遮挡 连续运动容易出现抖动 和 不稳定
% 为此 我们提出xxx的数据集xx包含spart view xxx pose,  以及动作内容相同的3D motion capture data from marked suit and multi-view MoCap system (Vicon)
% 我们的方法总述：构建xxx module，同时利用sparse-view 对齐但不一定合理的数据 和 动作准确合理但不一定对齐的数据，然后 xxx的优化
%In this paper, we tackle the above challenges and present \textit{ChallenCap} -- a template-based monocular 3D  capture approach for challenging human motions from a single RGB video, which outperforms existing state-of-the-art approaches significantly (See Fig.~\ref{fig:fig_1_teaser} for an overview). Our novel pipeline proves the effectiveness of embracing multi-modal references from both temporally unsynchronized marker-based system and light-weight markerless multi-view system in a data-driven manner, which enables robust human motion capture under challenging scenarios with extreme poses and complex motion patterns, whilst still maintaining monocular setup.
% 1 intro methods
%our ChallenCap utilizes a hybrid motion module learned with a weakly supervision from sparse-view estimated poses and the relevant MoCap data, and build an effective optimization with the priors of 2D/3D poses for accurate and reliable 3D poses,
% 2. Dataset
% To model this challenging motion capture problem in a data-driven manner, we collect a new Sparse-view Challenging Motion Capture (SCMC) dataset, which contains both video clips from four views as well as the corresponding relevant 3D motions captured via a motion capture system.

\section{Overview}
Our goal is to generate accurate bounding boxes for all objects of interests from a 3D scene, and describe each object with natural languages containing their location and attribute information.
%
Fig.~\ref{fig:overview} provides an overview of ChallenCap, which relies on a template mesh of the actor and makes full usage of multi-modal references in a learning-and-optimization framework.
%
Our method consists of a hybrid motion inference module to learn the challenging motion characteristics from the supervised references modalities, and a robust motion optimization module to further extract the reliable motion hints in the input images for more accurate tracking.
% A brief introduction of our main components is provided as follows.

\myparagraph{Template and Motion Representation.}
We use a 3D body scanner to generate the template mesh of the actor and rig it by fitting the Skinned Multi-Person Linear Model (SMPL)\cite{SMPL2015} to the template mesh and transferring the SMPL skinning weights to our scanned mesh.
%
The kinematic skeleton is parameterized as $\textbf{S}=[\boldsymbol{\theta}, \textbf{R},\textbf{t}]$, including the joint angles $\boldsymbol{\theta} \in \mathbb{R}^{30}$ of the $N_J$ joints, the global rotation $ \textbf{R}\in\mathbb{R}^3$ and translation $\textbf{t} \in \mathbb{R}^{3}$ of the root.
%
Furthermore, let $\textbf{Q}$ denotes the quaternions representation of the skeleton.
%
Thus, we can formulate $\textbf{S}=\mathcal{M}(\textbf{Q},\textbf{t})$ where $\mathcal{M}$ denotes the motion transformation between various representations.

% During motion inference, we design a novel network architecture, HybridNet, supervised via the references from both the unsynchronized marker-based and sparse multi-image systems. Note that the former marker-based reference encodes the accurate spatial motion characteristics but sacrifices the temporal consistency, while the latter multi-image reference provides overall 3D motion priors but fails to capture extreme poses.
% To avoid per-performer training and encode temporal motion information, we first obtain the initial noisy skeletal motion from monocular video as the input to our HybridNet.  
% Then, a novel loss or network XXXX


% 1. initial noisy skeletal motions --> quaternions motion map
% 2. GAN; encoder, decoder; multi-modal refernces
%  Temporal Encoder; Motion Discriminator
% 3. Dataset
\myparagraph{Hybrid Motion Inference.}
Our novel motion inference scheme extracts the challenging motion characteristics from the supervised marker-based and sparse multi-view references in a data-driven manner.
%
We first obtain the initial noisy skeletal motion map from the monocular video.
%
Then, a novel generation network, HybridNet, is adopted to boost the initial motion map, which consists of a temporal encoder-decoder to extract local and global motion details from the sparse-view references, as well as a motion discriminator to utilize the motion characteristics from the unpaired marker-based references.
%
To train our HybridNet, a new dataset with rich references modalities and various challenging motions is introduced (Sec. \ref{sec:mot_inference}).

% To tackle the monocular ambiguity and self-occlusion, we propose the hybrid motion module to model the feasible real world human poses for challenging video input via attention-based xxx network structure. Based on the prior of such hybrid motion poses, we further introduce this novel network to estimate the feasible poses from rough input so as to recover the reliable 3D motions. Our hybrid motion module consists of a attention-based xxx encoder, a xxx decoder to regress the poses from both global and local xxx (features), xxx to the 3D motion output . For weakly supervision, we formulate the xxx loss, the xxx loss, to train this hybrid motion net with the xx ability.


\myparagraph{Robust Motion Optimization.}
Besides the data-driven 3D motion characteristics from the previous stage, the input RGB video also encodes
reliable motion hints for those non-extreme poses, especially for the non-occluded regions.
%
Thus, a robust motion optimization is introduced to refine the skeletal motions so as to increase the tracking accuracy and overlay performance, which jointly utilizes the learned 3D prior from the supervised multi-modal references as well as the reliable 2D and silhouette information from the input image references (Sec. \ref{sec:mot_optimization}).

% For a challenging video input, we utilize the mentioned hybrid motion net to formulate an effective spatio-temporal optimization on the pose sequences. Based on a simple 3D pose estimator to produce the rough 3D poses input, We further propose this batch-based optimization, including xxx term and xxx, which enables stable and reliable 3D pose sequences for challenging motion captured with monocular camera.

% The following sections provide the details of the full system.



==> my_section/abstract.tex <==
\begin{abstract}
% 
\ct{3D dense captioning which localizes dense objects from a point cloud scene and describes each object with a sentence, has received increasing interest recently. Mainstream 3D dense captioning methods adopt an object proposal detector followed by a language captioner pipeline to do this task, where the object detector output has a heavy one-way impact on the captioner's performance with no communication between them, and the rich contexts beyond the detector's output in the scene are underestimated in the captioning process.  %achieves promising performance but are still insufficient faces insufficient contextual %
%pay much attention to relation modeling of object proposals, which successfully bridge the gap between scene understanding and natural language generation, however, these methods heavily depend on the detector.
Therefore, inspired by the success of Transformer models such as 3DETR for 3D vision tasks, we propose Scene2Cap, a scene-aware transformer-based 3D dense captioning approach to solve the above issues. Especially, a ** module is developed to fuse the context features extracted by ** with ** to achieve **. Then the captioner's output is feeback to the detector via ****, to achieve *** }
%
Extensive experiments on two commonly used datasets, ScanRefer and Nr3D, demonstrate that our approach can achieve ** accuracy than SOTA ** method under ** settings and scenarios.
%\textcolor{red}{[Ma: Should we mention the dataset in the abstract since it is one of our contribution?]}

\end{abstract}

==> my_section/cache.tex <==
\section{Introduction}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\linewidth]{fig/teaser.pdf}
	\caption{Two-stage models for 3D dense captioning vs. our proposed one-stage Vote2Cap-DETR.}
	\label{fig:teaser}
\end{figure}

% paragragh 1. Dense-Captioning on 3D scenes is important
3D dense captioning \cite{chen2021scan2cap,chen2021d3net,yuan2022x-trans2cap,wang2022spacap3d,jiao2022more,cai20223djcg} requires a system to localize all the objects in a 3D scene, and generate descriptive sentences for each object. 
%
Combining scene understanding with natural language generation, researches on 3D dense captioning benefit many applications such as natural language control in VR/AR systems and home appliance intelligence. 
%
This problem is challenging given 
%
1) the sparsity and occlusions of point clouds and
\csj{1) the uneven spatial distribution of objects and }
%
2) the cluttered and unbalanced distribution of object-caption pairs. 


% paragragh 2. our understanding of this task and issues
3D dense captioning can be divided into two tasks, object detection and object caption generation.
%
% Most existing works focus a few aspects of the pipeline. 
%
% First class: spatial relation modelling
%
Scan2Cap\cite{chen2021scan2cap}, MORE\cite{jiao2022more}, and SpaCap3D\cite{wang2022spacap3d} propose well-designed relation reasoning modules to efficiently model relations among object proposals.
%
\csj{And \cite{zhong2022contextual3DdenseCap} introducing a parallel branch to introduce additional contextual information.}
%
% Second class: joint training of grounding and captioning
%
3DJCG\cite{cai20223djcg} and D3Net\cite{chen2021d3net} study the correlation between 3D visual grounding and 3D dense captioning and point out that these two task promote each other.
%
% Third class: 2D to 3D knowledge transfer
%
Additionally, $\chi$-Trans2Cap\cite{yuan2022x-trans2cap} analyzes how to transfer knowledge from additional 2d information to boost 3d dense captioning.
%
Among all existing methods, they all adopt a two-stage “detect-then-describe” pipeline\cite{chen2021scan2cap,jiao2022more,wang2022spacap3d,cai20223djcg,chen2021d3net,zhong2022contextual3DdenseCap}.
%
It first generates a set of object proposals, then decode each object by a caption generator with explicit reasoning procedure.
%
Though outstanding performance have these methods achieved, the ``detect-then-describe'' pipeline suffers from following issues: 
%
1) Because of the serial and explicit reasoning, the performance highly depends on the object detection performance, which limits the mutual promotion of detection and captioning. 
%
2) The heavy reliance on hand-crafted components, e.g radii, 3D operators, definition of proposal neighbors, and post-processing(non-maximum suppression\cite{neubeck2006nms}) introduces additional hyper-parameters, leading to sub-optimal performance given the sparse object surfaces and cluttered object distributions among different indoor scenes.
%
Thus inspiring us toward a one-stage 3D dense captioning system.


To address the above issues, we propose Vote2Cap-DETR, a fully transformer encoder-decoder architecture for one-stage 3D dense captioning.
%
Instead of the traditional ``detect-then-describe'' pipeline, we directly feed the decoder's output into localization head and caption head in parallel.
%
By casting 3D dense captioning as a set-to-set problem, each target instance and its language annotation is matched to a query in a one-to-one correspondence, helping feature representation for proposals be more discriminative to identify each \textbf{distinctive} object from a 3D scene.
%
Additionally, we also propose a novel vote query driven decoder to introduce spatial bias for better localization of objects in a cluttered 3D scene.


With fully attentional design, we resolve the curse of 3D dense captioning with following three innovations: 
%
1) Our method consider the 3D dense captioning task as a set prediction problem. The proposed Vote2Cap-DETR directly decodes the features into an object sets with their locations and corresponding captions by applying two parallel prediction heads. 
%
2) we propose a novel vote decoder by reformulate the object queries in 3DETR into the format of the vote query that is a composition of the embeddings of the seeds point and the vote transformation of the box with respect to the seeds, which indicates the connection between the vote query in Vote2CAP-DETR with the VoteNet, but with better localization and higher training efficiencies; 
%
3) we develop a novel caption query driven head, which absorbs the relation and attribute modelling into the self- and cross-attnetion such that it can looks into both the local and global scene context to better describe.
%
Extensive experiments on two commonly used datasets, ScanRefer and Nr3D, demonstrate that our approach can achieve can surpass prior arts with many hand-craft procedures by large margin, which demonstrates the superiority of that fully transformer architecture with sophisticated vote head and caption head can inspire many 3D vision and language tasks. 

To summarize, the main contribution of this work include:
\begin{itemize} 
\setlength\itemsep{0em}
    \item We propose a novel one-stage and fully attention driven architecture for 3D dense captioning as a set-to-set prediction problem, which achieves a better balance between detection and captioning and narrows the gap between training and evaluation.

	\item Extensive experiments show that our proposed Vote2Cap approach achieves a new state-of-the-art performance on both Nr3D\cite{achlioptas2020referit3d}(-\% C@0.5) and ScanRefer\cite{chen2021scan2cap}(-\% C@0.5).
	
\end{itemize} 
